The functorial semantics of Lie theory

Ehresmann's introduction of differentiable groupoids in the 1950s may be seen as a starting point for two diverging lines of research, many-object Lie theory (the study of Lie algebroids and Lie groupoids) and sketch theory. This thesis uses tangent categories to build a bridge between these two lines of research, providing a structural account of Lie algebroids and the Lie functor. To accomplish this, we develop the theory of involution algebroids, which are a tangent-categorical sketch of Lie algebroids. We show that the category of Lie algebroids is precisely the category of involution algebroids in smooth manifolds, and that the category of Weil algebras is precisely the classifying category of an involution algebroid. This exhibits the category of Lie algebroids as a tangent-categorical functor category, and the Lie functor via precomposition with a functor $\partial: \mathsf{Weil}_1 \to \mathcal{T}_{\mathsf{Gpd}},$ bringing Lie algebroids and the Lie functor into the realm of functorial semantics.

==> Chapters/Ch5-InfNerve-Sanctuary.tex <==
\chapter{The infinitesimal nerve and its realization}%
\label{ch:inf-nerve-and-realization}




\section{Tangent categories via enrichment}%
\label{sec:tang-cats-enrichment}

This section demonstrates how tangent categories fit inside the framework of enriched categories. This connection  was first made by \cite{Garner2018}, building on the actegory perspective on tangent categories introduced in \cite{Leung2017} and a result relating monoidal actions and enrichment from \cite{Wood1978}. Garner was able to exhibit some of the major results from synthetic differential geometry as pieces of enriched category theory, for example the Yoneda lemma implies the existence of a well-adapted model of synthetic differential geometry.

The category of Weil spaces is the site of enrichment for tangent categories and are closely related to Dubuc's \emph{Weil topos} from his original work on models of synthetic differential geometry \cite{Dubuc1981}, and a deeper study of the topos may be found in \cite{Bertram2014}. Recall that the category $\wone$ is the free tangent category over a single object. The category of Weil spaces is the \emph{cofree} tangent category over $\s$, which is the category of transverse-limit-preserving functors $\wone \to \s$ by Observation \ref{obs:cofree-tangent-cat}. Call this the category of \emph{Weil spaces}, and write it $\w$. Just as a simplicial set $S: \delta \to \s$ is a gadget recording homotopical data, a Weil space is a gadget recording \emph{infinitesimal} data.

\begin{definition}%
	\label{def:weil-space}
	A \emph{Weil space} is a functor $\wone \to \s$ that preserves transverse limits - that is, the $\ox$-closure of the set of limits:
	\[
		\left\{
		\input{TikzDrawings/Ch5/wone-pb.tikz}
		,
		\input{TikzDrawings/Ch5/wone-univ-lift.tikz}
		,
		\input{TikzDrawings/Ch5/wone-id.tikz}
		\right\}
	\]
	A morphism of Weil spaces is a natural transformation. The category of Weil spaces is written $\w$.
\end{definition}
\begin{example}
	~\begin{enumerate}[(i)]
		\item Every commutative monoid may be regarded as a Weil space in a canonical way.
		      Observe that for every $V \in \wone$ and commutative monoid $M$, there is a free $V$-module structure on $M$ given by $|V| \ox_{\mathsf{CMon}} M$. The underlying commutative monoid of $V$ is exactly $\N^{\mathsf{\dim V}}$, so that:
		      \[
			      V \bullet M \cong \oplus^{\dim V} M
		      \]
		      The microlinearity of $V \mapsto |V| \ox M$ follows from fundamental properties of finite biproducts.
		\item Following (i), any tangent category $\C$ that is \emph{concrete} - it admits a faithful functor $U_\s: \C \to \s$ - will have a natural functor into tangent sets (copresheaves on $\wone$). Every object $A$ will have an underlying tangent set $V \mapsto U_{\s}(T^V(A))$, and whenever $U_\s$ preserves connected limits (such as the forgetful functor from commutative monoids to sets), each of the underlying tangent sets will be a Weil space.
		\item Consider a symmetric monoidal category with an infinitesimal object, which by Corollary \ref{cor:rewrite-rep-functor} is a transverse colimit preserving symmetric monoidal functor $D:\wone \to \C$. Then for every object, the nerve (Definition \ref{def:nerve}) $N_D(X): \C(D-,X):\wone \to \s$ is a Weil space.
		\item For any pair of objects $A,B$ in a tangent category, $\C(A,T^{(-)}B):\wone \to \s$ is a Weil space by the continuity of $\C(B,-):\C \to \s$.
	\end{enumerate}
\end{example}
Unlike the category of simplicial sets, the category of Weil spaces is not a topos.
The category of Weil spaces does, however, inherit some nice properties from the topos of copresheaves on $\wone$ by applying results from \Cref{sec:enriched-nerve-constructions}.
\begin{proposition}[\cite{Garner2018}]
	The category of Weil spaces is a cartesian-monoidal reflective subcategory of $[\wone,\s]$.
\end{proposition}
\begin{corollary}
	The category of Weil spaces is:
	\begin{enumerate}[(i)]
		\item A cartesian closed category.
		\item Locally finitely presentable as a cartesian monoidal category (as in Definition \ref{def:v-lfp})\footnote{
			      That is to say, the category of Weil spaces is a co-complete category with a dense subcategory $\yon:\wone \to \w$ (see Definition \ref{def:dense-subcat}).
		      }.
		\item A representable tangent category, where the infinitesimal object is given by the restricted Yoneda embedding $\yon: \wone^{op} \to \w$.
	\end{enumerate}
\end{corollary}
The cofree tangent structure on $\w$ is given by precomposition, that is:
\[
	T^U.M.(V) = M.(U \ox V) = M.T^U.V
\]
This tangent coincides with the representable tangent structure induced by the Yoneda embedding. The proof is an application of the Yoneda lemma. Observe:
\[
	[D,M](V) \cong [\wone,\s](D \x \yon(V), M) \cong [\wone, \s](\yon(WV), M) \cong M(WV)
\]
where $D \x \yon(V) = \yon(WV)$ as the tensor product in $\wone$ is cocartesian and the reflector is cartesian monoidal.

% Thus, we set the following piece of notation/terminology:
% \begin{notation}
% 	For a structure in a tangent category (e.g. a differential object, involution algebroid, etc), we call a model of $X$ in $\w$ a tangent $X$.
% \end{notation}

% % \paragraph{The enrichment of a tangent category in $\w$}%
% % \label{sub:enrichment-of-tang-cat}
% The basic idea in enriched category theory is that the definition of a category involves very little about the category of sets.
% Thus, we can define for any monoidal $\vv^\ox$ the notion of a $\vv$-category.


In general, any actegory over a monoidal $\C$ will give rise to $[\C,\s]$-enriched category, using the tensor structure induced by Day convolution, was proved by \cite{Wood1978}. \cite{Garner2018} showed that a monoidal reflective subcategory $\vv \hookrightarrow \hat \a$ exhibits the 2-category of $\vv$-categories as a reflective sub-2-category of $\a$-categories - this allow for tangent categories to be regarded as a particular class of enriched category.
\begin{proposition}[\cite{Garner2018}]
	Every tangent structure $(\C, \T)$ equips $\C$ with enrichment in Weil spaces.
\end{proposition}
\begin{proof}
	The presheaf is constructed:
	\[
		\underline{\C}(A,B) = \C(A, T^{}B): \wone \to \s
	\]
	The functor $\C(A,-)$ is continuous and $T^{-}B$ is a microlinear complex, so this is a Weil space. The following diagram gives the composition map :
	\input{TikzDrawings/Ch5/enrichment-in-W-comp.tikz}
	Note that it is natural in $U, V$.
\end{proof}
Enriched category theory introduces a new family of limits, \emph{powers}\footnote{Recall that the entire class of weighted limits is equivalent to conical (ordinary) limits and powers.}. Powers are essential in tangent category theory and satisfy a coherence due to \cite{LucyshynWright2016}.
\begin{definition}\label{def:power}
	Let $\C$ be a $\vv$-category for $\vv$ a closed symmetric monoidal category. For $J \in \vv$, the \emph{power} by $J$ for an object $C \in \C$ is an object $C^J$ so that the following is an isomorphism:
	\[
		\forall D: \vv(J, \C(D,C)) \cong \C(D,C^J)
	\]
	whereas the \emph{copower} is given by:
	\[
		\forall D: \vv(J, \C(C,D)) \cong \C(J \cdot C, D)
	\]
	Let $\j \hookleftarrow \vv$ be a full monoidal subcategory of $\vv$. A $\vv$-category $\C$ has \emph{coherently chosen powers} by $\j$ if there is a choice of $\j$-powers $(-)^J$ so that:
	\[
		(C^J)^K = C^{J \ox K}
	\]
	Moreover, coherently chosen copowers are a choice of $\j$-copowers so that:
	\[
		K \bullet (J \bullet C) = (K \ox J) \bullet C
	\]
	The sub-2-category of $\vv$-categories equipped with coherently chosen powers and copowers are $\vv\cat^\j$ and $\vv\cat_\j$, respectively.
\end{definition}

Now, returning to the specific enrichment in $\w$, remember that the hom-object between $A, B$ is given by:
\[
	V \mapsto \C(A,T^V B)
\]
For a representable functor $\yon U$, use the fact that the representable tangent structure induced by $\yon$ coincides with the cofree tangent structure and find:
\[
	\w(\yon U, V \mapsto \C(A, T^VB)) \cong V \mapsto \C(A, T^V.T^U(B))
\]
Then, a tangent category (and any actegory, really) does not simply have enrichment in $\w$; it also has coherently chosen powers by representable functors\footnote{The terms ``representable'' and ``representable functor'' will be used interchangeably in this thesis.}. $\w$-categories with coherently chosen powers by representables are \emph{exactly} tangent categories. Thus we have the following:
\begin{proposition}[\cite{Garner2018}]
	A tangent category is exactly an $\w$-category with coherently chosen powers by representables.
\end{proposition}
Now the original notions of (lax, strong, strict) tangent functors can be defined as $\w$-functors between $\w$-categories with coherently chosen powers, where the lax/strong/strict adjective now relates to the preservation of the coherently chosen powers.
\begin{theorem}[\cite{Garner2018}]\label{thm:2-cat-tangcat}
	We have the following equivalences of 2-categories.
	\begin{enumerate}[(i)]
		\item The 2-category of $\w$-categories with coherently chosen powers and $\mathsf{TangCat}_{\mathsf{Lax}}$
		\item The 2-category of $\w$-categories with coherently chosen powers and power-preserving $\w$ functors  and $\mathsf{TangCat}_{\mathsf{Strong}}$
		\item The 2-category of $\w$-categories with coherently chosen powers and chosen-power-preserving $\w$ functors $\mathsf{TangCat}_{\mathsf{Strict}}$
	\end{enumerate}
\end{theorem}
Note that the for a lax tangent functor $(F,\alpha): \C \to \D$, the map
\[
	\alpha.X: F.T.X \to T.F.X
\] can be seen as the unique morphism induced by universality. Conversely, for a strong tangent functor, the natural isomorphism $\alpha$ is the isomorphism from the power $F.T.X$ to the \emph{coherently chosen} power $T.F.X$, while a strict tangent functor preserves the coherent choice of powers.

The following observation is somewhat dual \Cref*{thm:2-cat-tangcat}, taking copowers by representables as the basic structure. It would be an unnecessary digression to develop the entire theory; however, it will be helpful to relate representable tangent structures.
\begin{observation}\label{obs:second-enrichment}
	Regard a cartesian category with an infinitesimal object $D$ (Definition \ref{def:inf-object}) as a $\w$-category, where copowers induce the enrichment (use that $D$ determines a functor $D:\wone \to \C$)
	\[
		\C(A,B):\wone \to \s := \underline{\C}(A \x D(-), B)
	\]
	Note, then, that a second infinitesimal object in $\C$, this time a monoidal $F: \wone^{op} \to \C$, may be regarded as an enriched functor \emph{for $D$'s enrichment} if there is monoidal natural transformation:
	\[
		d: D \Rightarrow F
	\]
	This natural transformation allows for the construction of the following map in $\w$ that is natural for $X \in \wone$:
	\[
		(X \mapsto \wone^{op}(U \x X,V)) \xrightarrow[]{F_{U\x X,V}} (X \mapsto \C(F.U\x F.X, F.V)) \xrightarrow[]{(id \x d)^*} (X \mapsto \C(F.U\x D.X, F.V))
	\]
	This exhibits $F$ as a $\w$-functor.
\end{observation}

As a final remark, note that the Yoneda lemma applies of $\w$-categories, so there is an embedding:
\[
	\C \hookrightarrow \widehat{C} = [\C^{op},\s]
\]
The powers and copowers by representables are computed pointwise in a presheaf category, so they inherit the coherent choice. Thus the following holds:
\begin{corollary}[\cite{Garner2018}]
	Every tangent category embeds into a $\w$-cocomplete representable tangent category.
\end{corollary}
(In fact, this result is the main theorem of \cite{Garner2018}).
\begin{corollary}
	The category of anchored bundles in a locally presentable tangent category is itself locally presentable, and in Weil spaces, the inclusion $\wone^* \hookrightarrow \mathsf{Anc}(\w)$ is a dense subcategory.
\end{corollary}



\subsection*{Differential bundles as enriched structures}%
\label{sub:differential-bundles-as-enriched-structures}

As a first case study using the enriched perspective for tangent categories, consider differential bundles. Most of the work in \Cref{ch:differential_bundles} uses the intuition that differential bundles were some tangent-categorical algebraic theory - this section will make that intuition concrete. Recall that a lift (Definition \ref{def:lift}) is a map $\lambda:E \to TE$. Using the enriched perspective treating $TE$ as a power (recall Definition \ref{def:power}), this gives the following correspondence:
\[
	\infer{\hat{\lambda}:D \to \C(E,E)}{\lambda: 1 \to \C(E, E^D)}
\]
The commutativity condition, then, is equivalent to asking that the following diagram commutes:
\[\input{TikzDrawings/Ch5/dbun-commutativity.tikz}\]
That is, $\hat{\lambda}$ is a semigroup morphism $D \to \C(E,E)$. In any cartesian closed category with coproducts, a semigroup may be freely lifted to a monoid using the "maybe monad" $(-) + 1$ from functional programming (see, for example, \cite{Seal2013}).
\begin{definition}%
	\label{def:lambda-monoid}
	Regard the following monoid the one-object $\w$-category $\Lambda$:
	\[
		\infer{m: (D+1) \x (D+1) \to D+1}{D \x D + D + D + 1 \xrightarrow{(\iota_L\o m | \iota_L | \iota_L |\iota_R)} D + 1}
	\]
\end{definition}
Thus, a lift $\lambda$ is exactly a functor from $\hat{\lambda}:\Lambda \to \C$. Now check that morphisms are tangent natural transformations.
\begin{lemma}%
	\label{lem:cat-of-lifts-iso}
	The category of lifts in a tangent category $\C$ is isomorphic to the category of $\w$-functors and $\w$-natural transformations $\Lambda^{op} \to \C$.
\end{lemma}
\begin{proof}
	Check that a $\w$-natural transformation is exactly morphism of lifts $f: \lambda \to l$. Start with the $\w$-naturality square:
	\[\input{TikzDrawings/Ch5/w-nat.tikz}\]
	Now, rewriting $D+1 \to \C(A,B)$ as a semigroup map $D \to \C(A,B)$, we have:
	\[
		\infer{
			\infer{
				1 \xrightarrow{Tf \o \lambda'}\C(A,TB)
			}{
				1 \xrightarrow{(\lambda',f)} \C(A,TA) \x \C(A,B) \xrightarrow{1 \x T} \C(A,TA) \x \C(TA,TB) \xrightarrow{m_{A,TA,TB}} \C(A,TB)
			}}{
			D \xrightarrow{(\lambda,f\o !)} \C(A,A) \x \C(A,B) \xrightarrow{m_{AAB}} \C(A,B)
		}
	\]
	Similarly, the other path is exactly $l \o f$. Thus, a $\w$-natural transformation is exactly a morphism of lifts.
\end{proof}
\begin{observation}
	The semigroup $D$ is commutative, so $\Lambda = \Lambda^{op}$ - the choice of using $\Lambda^{op}$ is to remain consistent with conventions used in \Cref{sec:enriched-nerve-constructions}.
\end{observation}
It is a classical result in synthetic differential geometry that the object $D$ has only one point - in the case of $\w$, this follows from the Yoneda lemma (regarding $\w$ as a $\s$-category)
\[
	\w(1,D) = \wone(\N[x]/x^2, \N) = \{ !: \N[x]/x^2 \to \N \}
\]
Note that this forces the natural idempotent $e:id \Rightarrow id$ from Proposition \ref{prop:idempotent-natural}, then, must be the point $0:1 \to D$. Note that this idempotent is an absorbing element of the monoid $D+1$, so for any $f:X \to D+1$, it follows that $m(f,0\o !) = m(0\o !, f) = 0\o !$.  A pre-differential bundle is exactly a lift with a chosen splitting of the natural idempotent $p\o\lambda$.
\begin{lemma}%
	\label{lem:splitting-of-idemp-is-lambdaplus}
	For every lift $\bar{\lambda}:\Lambda^{op} \to \C$, the natural idempotent $e = p \o \lambda$ is exactly
	\[1 \xrightarrow[]{0} D \xrightarrow[]{\iota_L} D+1 \to \C(E,E)\]
\end{lemma}
Now that the natural idempotent is a map in $\Lambda$, that idempotent splits to give the theory of a pre-differential object.
\begin{definition}%
	\label{def:lambda-plus}
	The $\w$-category $\Lambda^+$ is given by the set of objects $\{0,1\}$ with hom-Weil-spaces:
	\begin{itemize}
		\item $\Lambda^+(1,1) = D+1$, otherwise $\Lambda^+(i,j) = 1$.
		\item $m_{111} = m, m_{i11} = \iota_L \o 0 \o !, m_{i0j} = !$
	\end{itemize}
\end{definition}
% The following lemma lets simplifies the composition in $\Lambda^+$.
% \begin{lemma}
% 	Associativity of composition in $\Lambda^+$ can be written by embedding each hom-space into $D+1$
% 	$\w$-category, where we use inclusions:
% 	\begin{gather*}
% 		\Lambda^+(0,0) = 1 \xrightarrow{\iota_L \o 0 \o !} D+1  \hspace{0.25cm}
% 		\Lambda^+(0,1) = 1 \xrightarrow{\iota_L \o 0 \o !} D+1  \\
% 		\Lambda^+(1,0) = 1 \xrightarrow{\iota_L \o 0 \o !} D+1  \hspace{0.25cm}
% 		\Lambda^+(1,1) = D+1 \xrightarrow{id} D+1  
% 	\end{gather*}
%     \[\input{TikzDrawings/Ch5/assoc.tikz}\]
% \end{lemma}
Basic facts about idempotent splittings yield the following theorem:
\begin{lemma}%
	\label{lem:lambda-plus-is-pdb}
	The category of pre-differential bundles is exactly the category of $\w$-functors $(\Lambda^+)^{op} \to \C$ (that is, $\C$-valued presheaves).
\end{lemma}
($(\Lambda^+)^{op} = \Lambda^+$, so this is purely conventional).
It is straightforward to exhibit the category of differential bundles as a reflective subcategory of pre-differential bundles in $[(\Lambda^+)^{op}, \C]$ (so long as $\C$ has equalizers).
\begin{proposition}%
	\label{prop:Lambda-is-refl-subcat}
	The category of differential bundles in a tangent category $\C$ with $T$-equalizers and $T$-pullbacks is a reflective subcategory of $[(\Lambda^+)^{op}, \C]$, and is therefore a locally finitely presentable tangent category.
\end{proposition}
\begin{proof}
	The category of pre-differential bundles in $\C$ is isomorphic to $[(\Lambda^+)^{op}, \C]$. By Corollary \ref{cor:idemp-dbun}, the category of differential bundles is isomorphic to the category of algebras for a canonical idempotent monad on $\C$. The reflector sends a pre-differential bundle to the $T$-equalizer \input{TikzDrawings/Ch5/reflector.tikz}. This equalizer will always exist if $\C$ has equalizers, and pullbacks of the projection will exist if $\C$ has pullbacks, so the pullback is a differential bundle. This reflection gives a left-exact idempotent monad on $[(\Lambda^+)^{op}, \C]$ whose algebras are differential bundles.
\end{proof}
Now, in case $\C$ is a \emph{locally presentable} tangent category (such as $\w$), basic facts about locally presentable categories yields the following:
\begin{corollary}%
	\label{cor:Lambda-dense}
	If $\C$ is locally presentable, then $\mathsf{DBun}(\C)$ is a locally presentable category.
\end{corollary}
% \begin{corollary}
%     $\Lambda^+$ is a dense subcategory of differential bundles in $\w$. 
% \end{corollary}
% This corollary, the subcategory inclusion $\yon:\Lambda^+ \hookrightarrow \widehat{\Lambda^+}$ is dense in the category of differential bundles, means $\Lambda^+$ can act as the arities for a theory - this this case, the theory of anchored bundles.


\section{Enriched nerve constructions}%
\label{sec:enriched-nerve-constructions}

Nerve constructions present a powerful generalization of the Yoneda functor that sends an object $C \in \C$ to the representable presheaf $\C(-, C) \in \widehat{\C}$ (for reference material, see Chapter -- of \cite{Loregian2015}). %TODO add chapter
The Yoneda lemma states that this functor is an \emph{embedding} (that is, it is fully faithful), so no information is lost when embedding a category into its category of presheaves. 
Nerve constructions, then, move this towards an \emph{approximation} of the original category $\C$ by some subcategory $\D \hookrightarrow \C$, or more generally by some functor $K:\a \to \C$.

\begin{definition}%
	\label{def:nerve-of-a-functor}
		The \emph{nerve} of a $\vv$-functor $K: \a \to \C$ is the functor
	\[
		N_K: \C \to \widehat{\a}; \hspace{0.5cm} C \mapsto \C(K-, C)
	\]
	(where $\widehat{A}$ is the $\vv$-category of $\vv$-presheaves on small $\vv$-category $A$).
\end{definition}

\begin{example}%
	\label{ex:nerve-functors}
	~\begin{enumerate}[(i)]
		\item The nerve of the identity functor $\C = \C$ is the usual Yoneda embedding $\C \hookrightarrow \widehat{\C}$.
		\item 
		The first example of a nerve construction in the mathematical literature is the simplicial approximation of a topological space by \cite{Kan1958}.
		Recall the original construction of the simplicial nerve of a topological space $X$, where $X_n = \mathsf{Top}(\Delta_n,X)$.
		This is exactly the nerve of the functor $\bar{\Delta} \to \mathsf{Top}$ that sends $n$ to the $n$-simplex:
		\[
			\{
				x \in \R^n | \sum x_i = 1
			\}
		\]
		\item Recall that in -, a functor sending reflexive graphs to anchored bundles was constructed. This ``infinitesimal approximation'' of a reflexive graph may also be regarded as a nerve construction, first by looking at the category of reflexive graphs in $\w$, which is the presheaf category $[\mathsf{Refl}, \w]$ for the trivial category 
		\[
			blah % reflexive graph diagram
		\]
		This will be a representable tangent category, where $D$ is the disconnected graph $D = D$. By the Yoneda lemma, we have that:
		\[
			[\mathsf{Refl}, \w](\yon 1, G) = G_1,
			[\mathsf{Refl}, \w](\yon 0, G) = G_0,
			[\mathsf{Refl}, \w](D \x \yon(i), G) = T.G_i,
		\]
		So the limit diagram defining the infinitesimal approximation of a graph becomes:
		\[
			blah % TODO put the two graphs here	
		\]

		% \item The theory of locally finitely presentable categories gives a useful class of examples.
		%       Because we may represent a locally presentable $\C$ as $\mathsf{Lex}(\C_{fp}^{op}, \vv)$ (whenever $\vv$ itself is locally presentable as a closed category), we can see that the nerve of $\C_{fp} \hookrightarrow \C$ is a fully faithful functor, and the realization is the reflection from presheaves on $\C_{fp}$ to models.
		% \item In general, a tangent category $\C$ is locally finitely presentable whenever it is the reflective subcategory of $\widehat{\a}$ for some small $\w$-category $\a$ - if the representables $\a \hookrightarrow \widehat{\a}$ belong to $\C$, then the inclusion $\C \hookrightarrow \widehat{\a}$ is induced by the nerve of $\a \hookrightarrow \C$.
	\end{enumerate}
\end{example}

Recall that the simplicial localization in \cite{Kan1958} has a left adjoint, the \emph{geometric realization}, that constructs a topological space using the data of a simplicial set. 
This realization may be constructed using a left Kan extension.
\begin{definition}%
	\label{def:realization}
	Let $K: \a \to \C$ be a $\vv$-functor for a cocomplete $\C$.
	The \emph{realization} of $K$ is the left Kan extension:
	\[
		\input{TikzDrawings/Ch5/realization.tikz}
		\hspace{0.5cm}
		|C|_K := \int^A \C(KA, C) \cdot KA
	\]
	A \emph{nerve/realization context} is $\vv$-functor $K:\a \to \C$ from a small $A$ to a cocomplete $\C$.   
\end{definition}
The adjunction between simplicial sets and topological spaces fits into general categorical machinery as a nerve/realization context.
\begin{lemma}
	For every nerve/realization context $K: \a \to \C$, the realization of $K$ is left adjoint to the nerve of $K$.
\end{lemma}

% Note that in Example \ref{ex:blah}, each of the approximations above loses some data (except for the identity functor). It will be useful to identify those functors $K: \a \to \C$ whose nerve behaves like the Yoneda embedding - that is, they are fully faithful. This condition is known as \emph{density}, and is explored in Chapter 5 of \cite{Kelly2005}.

% \begin{definition}%
% 	\label{def:dense}
% 	A functor $K: \a \to \C$ is \textit{dense} whenever its nerve:
% 	\[
% 		N_K: \C \to \widehat{A}; C \mapsto \C(K-,C)	
% 	\]
% 	If $K$ is a subcategory inclusion, we call this a \emph{dense subcategory}.
% \end{definition}

% \begin{example}
% 	\begin{itemize}
% 		\item For any small category $\C$, the identity functor $\C = \C$ is dense, as is the Yoneda embedding $\yon: \C \to \widehat{\C}$ is a dense functor. 
% 		\item The category of finite sets is a dense subcategory of $\s$, it follows that the category of finite cardinals - that is, the full subcategory of sets whose objects are $[n] = \coprod_n 1$ - is a dense subcategory of $\s$.
% 		\item Recall that a monad on $\s$ is a
% 	\end{itemize}
% \end{example}
% \begin{itemize}
% 	\item Nerve constructions are a powerful generalization of the Yoneda embedding that sends an object $C$ to the presheaf $\C(-, C)$.
% 	\item The Yoneda lemma states that the functor assigning a an object to its representable presheaf is \emph{fully faithful} (i.e. an embedding) - so it completely preserves the data of the category.
% 	\item Nerve constructions, then, move towards \emph{approximations} of the original category by a small subcategory, or more generally by a functor from some small subcategory $K: \a \to \C$.
% 	\item Definition of nerve here.
% 	\item Example: (simplicial localization, sets + Nats, Signpost towards the infinitesimal approximation using reflexive graphs)
% 	\item Parenthetical remark about how it's unclear where the ``nerve'' language came from - but it seems that Kan's original ``simplicial approximation'' captures the intuition most clearly, but in the interest of connecting to the relevant literature we stick to their language.
% 	\item Next, talk about \emph{density} - this determines when a category is completely approximated by a functor.
% 	% \item A first step towards a nerve construction is to think about subcategories - for example, one consequence of the Yoneda lemma is that every presheaf may be written as the coend:
% 	% \item If one wanted to ``aprox''
% 	\item Some neat little results. 
% 	\item Example: the anchored bundle one.
% \end{itemize}



% % The nerve construction 
% % This section gives a short review the \emph{nervous theories} paradigm of \cite{Bourke2019}, along with the \emph{nerve/realization} contexts of \cite{Kan1958} (a recent exposition may be found in \cite{Loregian2015}).The common denominator here is the notion of a nerve. The ``nerve'' of an internal category and involution algebroid were discussed in \Cref{sec:weil-nerve}, although the notion of a nerve or Segal condition was not made precise.
% \begin{definition}%
% 	\label{def:nerve}
% 	The \emph{nerve} of a $\vv$-functor $K: \a \to \C$ is the functor
% 	\[
% 		N_K: \C \to \widehat{\a}; \hspace{0.5cm} C \mapsto \C(K-, C)
% 	\]
% 	(where $\widehat{A}$ is the $\vv$-category of $\vv$-presheaves on small $\vv$-category $A$).
% 	Whenever $\C$ is cocomplete, the nerve has a left adjoint called the \emph{realization}, computed by the left Kan extension/coend:
% 	\[
% 		\input{TikzDrawings/Ch5/realization.tikz}
% 		\hspace{0.5cm}
% 		|C|_K := \int^A \C(KA, C) \cdot KA
% 	\]
% 	A \emph{nerve/realization context} is $\vv$-functor $K:\a \to \C$ from a small $A$ to a cocomplete $\C$.
% \end{definition}
% % We can see that the nerve itself may be represented as a left Kan extension:
% % \begin{lemma}
% \begin{observation}
% 	The nerve functor itself is equivalently the left Kan extension of $K$ along $\yon$:
% 	\[\input{TikzDrawings/Ch5/nerve-is-lany.tikz}\]
% 	For proof, see \cite{Loregian2015}. This presentation gives the unusual property that the nerve/realization adjunction is of the form:
% 	\[
% 		Lan_{\yon}K \vvdash Lan_K\yon
% 	\]
% \end{observation}

% \begin{example}
% 	~\begin{enumerate}[(i)]
% 		\item Recall the original construction of the simplicial nerve of a topological space $X$, where $X_n = \mathsf{Top}(\Delta_n,X)$.
% 		      This is exactly the nerve of the functor $\bar{\Delta} \to \mathsf{Top}$ that sends $n$ to the $n$-simplex:
% 		      \[
% 			      \{
% 			      	x \in \R^n | \sum x_i = 1
% 			      \}
% 		      \]
% 		\item The theory of locally finitely presentable categories gives a useful class of examples.
% 		      Because we may represent a locally presentable $\C$ as $\mathsf{Lex}(\C_{fp}^{op}, \vv)$ (whenever $\vv$ itself is locally presentable as a closed category), we can see that the nerve of $\C_{fp} \hookrightarrow \C$ is a fully faithful functor, and the realization is the ref$lection from presheaves on $\C_{fp}$ to models.
% 		\item In general, a tangent category $\C$ is locally finitely presentable whenever it is the reflective subcategory of $\widehat{\a}$ for some small $\w$-category $\a$ - if the representables $\a \hookrightarrow \widehat{\a}$ belong to $\C$, then the inclusion $\C \hookrightarrow \widehat{\a}$ is induced by the nerve of $\a \hookrightarrow \C$.
% 	\end{enumerate}
% \end{example}

% The situation where the nerve of $K$ is fully faithful is particularly important - Kelly called these functors \emph{dense}, by metaphor with the notion of density found in Hausdorff spaces. A dense subcategory models the same situation, except we replace ``continuous functions'' with ``co-continuous functors''. That is to say, a functor $K:\a \to \c$ into a cocomplete $\c$ is \textit{dense} whenever each object $C \in \c_0$ is canonically written as a coend:
% \[
% 	\int^A \C(KA, C)\cdot KA
% \]
% so that a cocontinuous functor $F:\c \to \d$ is determined by $F.K$.
% The general definition of density does not require a cocomplete category.
% \begin{definition}%
% 	\label{def:dense}
% 	A functor $K: \a \to \C$ is \textit{dense} whenever one of the following conditions holds
% 	\begin{itemize}
% 		\item The identity functor $id:\C \to \C$ is the left Kan extension of $K$ along itself, so: $Lan_K K = id$.
% 		\item Every object is given as the weighted colimit $C = N_K(C) \star K$.
% 		\item The nerve of $K$ is fully faithful.
% 	\end{itemize}
% 	Note that a locally finitely presentable category is precisely\footnote{Assuming that Vopenka's principle holds \cite{Adamek1994}.}
% 	 a cocomplete category $\C$ with a dense functor $K: \a \to \C$.
% \end{definition}
% Dense functors are poorly behaved under composition, but there is a useful cancellativity results from Chapter 5.2 of \cite{Kelly2005}.
% \begin{proposition}
% 	Consider a diagram of $\vv$-categories
% 	\[\input{TikzDrawings/Ch5/lan-result.tikz}\]
% 	where $\alpha$ is a natural isomorphism, and $K$ is dense.
% 	If this diagram exhibits $(\alpha, J)$ as the left Kan extension of $K$ along $F$, then $J$ is dense.
% \end{proposition}
% \begin{corollary}%
% 	\label{cor:dense-ff-result}
% 	If $K$ is dense, $F$ is fully faithful, and  $J.F = K$, then $F$ is a dense subcategory.s
% \end{corollary}
% Generally speaking, we will often refer to dense \textit{subcategories} rather than dense \textit{functors}. Through a naive application of the (bo,ff)-factorization system on $\vv$-categories, every dense functor induces a dense subcategory, as $K$ factors as
% \[
% 	K = \a \xrightarrow[]{K'} \mathsf{im}(K) \hookrightarrow \C
% \]
% so the inclusion of $\mathsf{im}(K)$ into $\C$ is dense.
% % \begin{proposition}
% % 	Let $K:A \to \c$ be a dense functor. Then the full subcategory $im(K)$ is a dense subcategory.
% % \end{proposition}
% % \begin{proof}
% % 	Use Corollary \ref{cor:dense-ff-result}.
% % \end{proof}
% % \begin{example}
% % 	Consider the category of transverse-limit preserving copresheaves of $\wone$ algebras $\w = \mathsf{Mod}(\wone, \s)$, the category of Weil spaces. We have the following dense subcategories:
% % 	\begin{enumerate}
% % 		\item The unit: $K_1: 1 \hookrightarrow \w$
% % 		\item The infinitesimals: $D: \wone^{op} \hookrightarrow \w$
% % 		\item The finite-coproduct closure of infinitesimals $\{ \sum D_v | v \in \wone \} \hookrightarrow \w$ 
% % 	\end{enumerate} 
% % \end{example}
% The category of finite sets is dense in $\s$, as $\s$ is locally finitely presentable, and the finitely presentable sets are exactly finite sets. In particular, this means that the skeleton of finite sets, where each object is $[n] = \{1, \dots, n\}$, is dense in $\s$.  A dense subcategory $\a$ of $\C$, then, acts as a generalization of this context - the objects $A \in \a$ may act as the \emph{arities} for a theory in $\C$.


% % \subsection*{Anchored bundles are concrete models of a $\Lambda^+$-theory}

% % Anchored bundles provide a good first application of nervous theories to tangent categories. Recall that an anchored bundle is a differential bundle $(\pi:A \to M, \xi, \lambda)$ equipped with an anchor map $\anc: A \to TM$. Regarding a differential bundle as a functor $\Lambda^+ \to \C$ (Proposition \ref{prop:Lambda-is-refl-subcat}), this corresponds to a natural transformation:
% % \[\input{TikzDrawings/Ch5/anc-as-nat.tikz}\]
% % Now, it is always the case that $TM$ is the power $M^{D}$, so a reasonable first step is to find a category $\mathsf{Anchor}$ so that there is a bijective on objects functor $\Lambda^+ \to \mathsf{Anchor}$ that sends $1$ to a cone for $T.0$ - this would induce an anchor map as follows:
% % \[\input{TikzDrawings/Ch5/anc-as-nat-2.tikz}\]
% % The obvious solution works best in this case - take some full subcategory of $\w$.
% % \begin{definition}%
% % 	\label{def:truncated-wone}
% % 	A Weil algebra has \emph{width} $k \in \N$ if it is written:
% % 	\[
% % 		V = \ox^{0 \le i < k} W_{n(i)}, n(i) \in \N
% % 	\]
% % 	The category of $k$-truncated Weil algebras, written $\wone^k$, is the full $\w$-subcategory of $\wone$ of Weil algebras of width $k$ or less.
% % \end{definition}
% % Note that for each $V$ in $\wone^k$, the enrichment is given by:
% % \[
% % 	\wone^k(U,V) := (X \mapsto \underline{\wone}(U, X \ox V) )
% % \]
% % The maps in $\wone^1$ - that is, the full subcategory of $\wone$ spanned by:
% % \[
% % 	\N, W, W_2, \dots
% % \]
% % has a useful property:
% % \begin{lemma}\label{lem:writing-maps-in-wone}
% % 	Every morphism:
% % 	\[
% % 		W_n \to V \in \wone
% % 	\]
% % 	may be written using only $\{p,+,0,\ell\}$ (closed under $\ox, \o$ and maps induced by transverse limits).
% % \end{lemma}
% % \begin{proof}
% % 	This is a consequence of the fact that every map $W_n \to V$ in $\wone$ may be written:
% % 	\[
% % 		v \mapsto \sum_{x} (A_x v)\cdot x
% % 	\]
% % 	where $x \in \mathsf{var}(V)$, and $A_x$ is in $\N^n$ so that $A_n v$ is the ordinary dot product.
% % 	Each individual term may be formed without $c$, and the whole term is then constructed by adding each component using the appropriate $U.+.V$-symbols. (This may also be regarded as a consequence of the graphical notation for maps in $\wone$ in Table 1 on page 308 of \cite{Leung2017}.)
% % \end{proof}
% %  It is possible, then, to show that the category of anchored bundles in $\C$ is a full sub-tangent-category of functors $\wone^1 \to \C$ - note that $W$ acts as a cone for $(-)^{\yon(W)}$, so this induces a map:
% % \[
% % 	\anc: F(W) \to T.F(\N)
% % \]
% % \begin{proposition}
% % 	\label{prop:nerve-anc-work}
% % 	Every anchored differential bundle in $\C$ determines a functor $\wone^1 \to \C$; a morphism is exactly a tangent natural transformation.
% % \end{proposition}
% % \begin{proof}
% % 	Start with an anchored bundle $(q:E \to M, \xi, \lambda, \anc)$, then for hom-objects with domain $\N$:
% % 	\[
% % 		\wone^1(\N,\N) = 1 \mapsto id_M \hspace{0.5cm} \wone^1(\N,T) = 1 \mapsto \xi
% % 	\]
% % 	The hom-objects with domain $T$, the problem is slightly more difficult, as $\wone^1(T,\N)(T^V) = \wone(T, T^V)$ and $\wone^1(T, T)(T) = \wone(T, T.T^V)$. This part of the  proof amounts to constructing maps:
% % 	\[
% % 		\wone(T, T^V) \to \C(E, T^V.M) \hspace{0.5cm}  \wone(T,T^V.T) \to \C(E, T^V.E)
% % 	\]
% % 	The first mapping is straightforward, send $\theta$ to $\theta.M \o \anc$. For the second map, observe that the following diagrams commute:
% % 	\[
% % 		\input{TikzDrawings/Ch5/anc-atlas.tikz}
% % 	\]
% % 	The idea, then, is to take $f$ and rewrite it as a string of compositions that does not include $c$ and switch out every occurrence of
% % 	\[
% % 		T^V.\theta.M, \theta \in \{p,0,+,\ell\}
% % 	\]
% % 	replace it with $T^V.(\theta')$, where $\theta'$ is the corresponding map in $\{q,\xi,+_q,\lambda\}$. This induces a map $\wone^1(W,W) \to \C(E,E) \in \w$, and the $\anc$ is exactly the unique $\alpha: F.W \to T.F$ induced by universality.

% % 	For morphisms, the inclusion $\Lambda^+ \to \wone$ ensures that any tangent natural transformation will be a linear morphism on the underlying differential bundle, and the tangent natural transformations coherences ensures that a tangent natural transformation will preserve the anchor. Conversely, an anchored bundle morphism will preserve each of the constructed morphisms $E \to T^V.E, E \to T^V.M$ (as it preserves each of $\{ q, +_q, \xi, \lambda\}$), giving a tangent natural transformation. Thus there is a faithful embedding $\mathsf{Anc}(\C) \hookrightarrow [\wone^1, \C]$.
% % \end{proof}
% % Now restrict to the category $\wone^*$, the full subcategory of $\wone$ spanned by $\{\N, W\}$, the density result \Cref{cor:dense-ff-result} yields the following.
% % \begin{corollary}%
% % 	\label{cor:dense-subcat}
% % 	The category of anchored bundles is a full subcategory of $[{\wone^*},\C]$.
% % \end{corollary}
% % Observe that there is a bijective-on-objects functor
% % \[
% % 	a: \Lambda^+ \to \wone^*
% % \]
% % The category $\Lambda^+$ is a dense subcategory of differential bundles, and each object $\N, 1$ have the structure of a differential bundle.
% % \begin{lemma}
% % 	The category $\wone^1$ is a $\Lambda^+$-theory on the category of differential bundles in $\w$.
% % \end{lemma}
% % The category of anchored bundles in $\w$ is the category of presheaves on $(\wone^{1})^{op}$ whose underlying pre-differential bundle is a differential bundle. Thus we characterize the category of anchored bundles as a following pullback in $\w\mathsf{CAT}$.
% % \begin{proposition}\label{prop:models-in-C-anc}
% % 	The category of anchored bundles in $\C$ is equivalent to the pullback of $\w$-categories:
% % 	\[\input{TikzDrawings/Ch5/anc-as-pb-in-cat2.tikz}\]
% % \end{proposition}
% % \begin{proof}
% % 	A functor $\wone^* \to \C$ is an anchored bundle precisely whenever $\Lambda^+ \to \wone^* \to \C$ is a differential bundle, and the uniquely induced map:
% % 	\[
% % 		\hat A.W \to T.\hat A.\N	
% % 	\] gives the anchor map (naturality ensures linearity). Fully faithfulness was proved in \Cref*{prop:nerve-anc-work}.
% % \end{proof}
% % Now restricting to Weil spaces, the diagram:
% % \[\input{TikzDrawings/Ch5/anc-as-pb-in-cat.tikz}\]
% % yields the following corollary.
% % \begin{corollary}\label{cor:models-in-w-anc}
% % 	Anchored bundles are monadic over differential bundles in $\w$.
% % \end{corollary}
% % This result gives a Segal condition for anchored bundles, although it is quite simplistic: a $\w$-functor $A:\wone^1 \to \C$ is an anchored bundle if and only if $A.a:\Lambda^+ \to \C$ is a differential bundle.

\section{Nervous Theories}%
\label{sec:nervous_theories}

\begin{itemize}
	\item Lifting the characterization of algebroids from Theorem \ref{thm:weil-nerve} to the enriched perspective introduces the challenge of finding the appropriate framework to describe them.
	\item A natural candidate would be Kelly's enriched sketches, which are small $\vv$-categories equipped with a chosen class of limit cones - however there is no simple way to require the natural part $\alpha: F.T \Rightarrow T.F$ is cartesian when $\alpha$ is the map induced by a choice of weighed limit.
	\item The nervous theories of \cite{Bourke2019} provide a natural generalization of -, where blah is an anchored bundle and blahhh 
\end{itemize}

\begin{itemize}
	\item Nervous theories are generalizations of Lawvere theories, which here are product-preserving functors:
	\item Models of Lawvere theories are, of course, strictly product preserving functors. But they may also be thought of as functors $\th \to \s$ so that $\Sigma^{op} \o \th \to \s$ is strictly product-preserving - that means, it must be the nerve of $A$ for blah
	\item This generalizes as follows:
\end{itemize}

Then: 
\begin{itemize}
	\item original exposition on theories.
	\item add the comodel stuff.
\end{itemize}
% Recall that a Lawvere theory is a bijective-on-objects, product-preserving functor:
% \[
% 	\mathsf{FinSet_{Skel}} \to \mathbb{T}
% \]
% There is a generalized notion of Lawvere theory based on the idea that a dense subcategory can play the role of $ \mathsf{FinSet_{Skel}}$. \cite{Power1999} was the first to extend this to an arbitrary $\vv$-LFP $\C$, where the arguments for a Lawvere theory over $\C$ would then be the finitely presentable objects $\C_{fp}$. \cite{Berger2012} generalized this to dense subcategories of $\s$-LFPs $\C$, and Garner-Bourke's paradigm moved to dense sub-$\vv$-categories of LFP $\vv$-categories, and the presentation in this section follows the refinement of these ideas in \cite{Bourke2019}.

% \begin{definition}%
% 	\label{def:nerve-theory}
% 	Let $K:\a \to \C$ be a dense $\vv$-subcategory of a locally finitely presentable $\c$. We call the replete image of $N_K$ in $\widehat{\a}$ the category of $K$-nerves. An \textit{$\a$-theory} is a bijective-on-object $\vv$-functor $J: \a \to \th$, where each
% 	\[
% 		\th(J-,a): \a \to \vv
% 	\] is a $K$-nerve.
% 	The category of concrete models for an $\a$-theory is given by the pullback in $\vv\mathsf{CAT}$:
% 	\[\input{TikzDrawings/Ch5/conc-models.tikz}\]
% 	We say that an $\a$-presheaf $X$ satisfies the $K$-Segal conditions whenever $t^*X$ is a $K$-nerve (that is, it is a concrete model of the theory).
% \end{definition}
% \begin{example}
% 	~\begin{enumerate}[(i)]
% 		\item A functor $t:\mathsf{FinSet_{Skel}} \hookrightarrow \th$ is a $\mathsf{FinSet_{Skel}}$-theory if and only if $\th$ is a Lawvere theory. The Segal conditions in this case identify the models of the Lawvere theory.
% 		\item The inclusion of $\mathsf{Pth} \hookrightarrow \Delta$ is a $\mathsf{Pth}$-theory for the category of graphs. The Segal conditions in this case capture the classical Segal conditions for categories.
% 	\end{enumerate}
% \end{example}
% \cite{Bourke2019} give an idempotent adjunction between pre-theories and monads over a category, that is refined to an equivalence of categories between theories and \emph{nervous} monads. For the purposes of this thesis, the following suffices:
% \begin{proposition}
% 	Let $K: \a \hookrightarrow \C$ be a dense $\vv$-subcategory, and $J: \a \to \th$ an $\a$-theory.
% 	The category of concrete models of $J$ is monadic over $\C$.
% \end{proposition}
% \begin{proof}
%     This proof relies on a technical lemma - note that $N_K$ is fully faithful and monadic (as it is the inclusion of full reflective subcategory), and $J^*$ is monadic as $J$ is a bijective-on-objects functor. The pullback along $N_K$ will be fully faithful (as fully faithful functors are the right class of maps for the (bo,ff)-factorization system on $\vv$-categories). 
% \end{proof}

\section{The Weil nerve and Segal conditions for involution algebroids}%
\label{sec:revisiting-segal-conds}

This section proves one of the main theorems of this thesis - the category of algebroids is algebraic. That is, the category of involution algebroids is algebraic over the category of anchored bundles. \cite{Kapranov2007} showed that something like this held in the category of vector bundles over a smooth manifold, if the vector bundles are allowed to be infinite-dimensional. All of the actual work to prove this theorem was completed in \Cref{chap:weil-nerve}, particularly by Theorem \ref{thm:weil-nerve,cor:the-prolongation-description}.

% \begin{itemize}
	
% \end{itemize}


In $\mathsf{Gph}(\s)$, the path complex at $n$ for a graph is given by a choice of pullback
\[\input{TikzDrawings/Ch5/graph-comp.tikz}\]
This is represented by the following pushout:
\[ \input{TikzDrawings/Ch5/dense-in-graphs.tikz}\]
A construction of this flavour works for any ``co-graph'' in a category $\C$, so that the nerve of the co-graph lands in graphs, and the nerve of the path-complex sends the graph $N\dots$ to its path complex. Repeating this for the Weil nerve then requires a notion of a co-anchored bundle and its co-prolongation - however, all of the necessary results from \Cref{sec:weil-nerve} translate over by duality.

\begin{definition}%
	\label{def:coanc-bundle}
	Let $\C$ be a $\w$-category with coherently chosen copowers by representables (so that $\C^{op}$ is a tangent category). A \emph{co}-anchored bundle in $\C$ is an anchored bundle in $\C^{op}$.
	\begin{enumerate}[(i)]
		\item A co-differential bundle, so a triple:
		      \[
			      (y:D \cdot L \to L, q:M \to L, \xi:L \to M)
		      \]
		      so that $y$ is a semigroup action:
		      \[\input{TikzDrawings/Ch5/semigroup-action.tikz}\]
		      and $q \o \xi$ splits the idempotent $e = y \o (0\o !, id)$ and the following diagram is a coequalizer:\[\input{TikzDrawings/Ch5/coeq-coanc.tikz}\]
		      and pushout powers $L(n)$ of $q:M \to L$ exist and are preserved by $D \x (-)$.
		\item There is a co-anchor: a map $d:D\x M \to L$ so that
		      \[\input{TikzDrawings/Ch5/coanc.tikz}\]
	\end{enumerate}
\end{definition}
This definition has an immediate consequence, as $\C(-, A):\C^{op} \to \w$ is continuous for every $A \in \C$ (so it sends colimits in $\C$ to limits in $\w$). (It is important to remember here that powers in $\C$ are copowers in $\C^{op}$, and vice versa).
\begin{lemma}%
	\label{lem:nerve-of-coanc}
	Let $\C$ be $\w$-category with coherently chosen copowers by representables.
	For any co-anchored bundle $K: (\wone^*)^{op} \to \C$, the nerve of $K$ lands in anchored bundles in $\w$.
	\[
		N_K: \C \to \mathsf{Anc}(\w)
	\]
\end{lemma}

The construction of the co-prolongations of a co-differential bundle is dual to the prolongations from Definition \ref{def:prolongation-of-anchored-bundle} (where span composition is replaced with the dual notion of \emph{cospan} composition).
\begin{definition}%
	\label{def:coprol}
	Let $(y:D \cdot L \to L, q:M \to L, \xi:L \to M)$ be a co-anchored codifferential bundle in a $\w$-category with an coherently chosen copowers by representables. The coprolongation of $A$ by a Weil algebra $V$ is the cospan defined by the dual of $\boxtimes$, written $\boxplus$. So for cospans of the form:
	\[
		M \xrightarrow[]{l_X} X \xleftarrow[]{r_X} D_U \cdot M,
		M \xrightarrow[]{l_Y} Y \xleftarrow[]{r_Y} D_V \cdot M
	\]
	The cospan $(X:M \to D_U \cdot M)\boxplus (Y:M \to D_V\cdot M)$ is given by the pushout:
	\[\input{TikzDrawings/Ch5/cospan-compuv.tikz}\]
	% \begin{enumerate}[(i)]
	%     \item $L_{\N}: M \xrightarrow{=} M \xleftarrow{=} M$
	%     \item $L_{W_n}:1 \xrightarrow{\prod^n q} L(n) \xleftarrow{\delta(n)} D(n)$
	%     \item $L_{UV}$ is given by cospan composition:
	%     \[\input{TikzDrawings/Ch5/cospan-comp.tikz}\]
	% \end{enumerate}
	Then for any $V = W_{n(1)} \ox \dots \ox W_{n(k)}$, the object $L_V$ is the apex of the cospan:
	\[
		L_V := L(n_1) \boxplus \dots \boxplus L(n_k)
	\]
	This pushout is the \emph{$V$-coprolongation} of $L$.
\end{definition}
\begin{example}
	The $V$-coprolongation of the infinitesimal object $D$ in a representable tangent category is $D_V$.
\end{example}
The following results follow by duality.
\begin{proposition}%
	\label{prop:coanc-facts}
	Let $(y:D \cdot L \to L, q:M \to L, \xi:L \to M)$ be a co-anchored codifferential bundle in a $\w$-category with an coherently chosen copowers by representables. Then
	\begin{enumerate}
		\item There is a co-additive bundle $(q:M \to L, \xi:L \to M, \delta_L:L \to L(2))$, and $d$ is a co-additive bundle morphism.
		\item There is a morphism $\boxdot: L \boxplus L \to L$ (\Cref{def:coprol}), defined:
		      \[
			      L \po{d}{D \cdot q} D \cdot L \xrightarrow[]{(e | y)} L
		      \]
		\item The following diagram is a coequalizer.
		      \[
			      \input{TikzDrawings/Ch5/coanc-couni.tikz}
		      \]
	\end{enumerate}
\end{proposition}

Now, consider the co-anchored bundle induced by the fully faithful functor:
\[
	\yon: \wone^* \to \mathsf{Anc}(\w)
\]
So in this case, $L_V$ represents the functor that sends an anchored bundle $A$ to $\prol(V,A)$. Furthermore, $d:D \to L$ is the unique map induced by the couniversality of $D$. Now define the following.
\begin{definition}%
	\label{def:prol-cat}
	Define the full subcategory of $\mathsf{Anc}(\w)$ spanned by $L_V, V \in \wone$, to be $\prol$. Furthermore, write the full subcategory of $\mathsf{Anc}(\w)$ spanned by $V \in \wone^k$ as $\prol^k$.
\end{definition}
\begin{proposition}%
	\label{prop:nerve-thm-for-coprol}
	Every anchored bundle with chosen prolongations in a tangent category $\C$ determines a $\w$-functor $\prol^{op} \to \C$, and the embedding of $\mathsf{Anc}^* \to [\prol^{op}, \C]$ is fully faithful.
\end{proposition}

The category $\prol$, then, will play the role of the arities for involution algebroids, which is unsurprising based on the wording of Corollary \ref{cor:the-prolongation-description}. The construction of the functor:
\[
	w: \prol \to \wone^{op}
\]
is surprisingly straightforward.
\begin{observation}
	Recall that for any tangent category $\C$, Proposition \ref{prop:c-refl-in-anc} states that the category $\C$ is a reflective subcategory of $\mathsf{Anc}(\C)$. Because the reflection sends $A \mapsto TM$, it will map $L \mapsto D$ - then it must map:
	\[
		L_V \mapsto D_V
	\] as the coprolongation of $D_V$ for the co-anchored bundle $D$ is $D_V$, and left adjoints preserve colimits. This reflection restricts to a functor:
	\[
		\prol \to \wone^{op}
	\]
	Note that this sends $\boxplus^k_{i=1} L(n_i) \mapsto \prod^k_{i=1}D(n_i)$.
\end{observation}

\begin{theorem}%
	\label{thm:pullback-in-cat-of-cats-inv-algd}
	The category of involution algebroids with chosen prolongations in a tangent category $\C$ is precisely the pullback in $\w\mathsf{CAT}$:
	\begin{equation}\label{eq:prol2}
		\input{TikzDrawings/Ch5/prol2.tikz}
	\end{equation}
	where $w$ is the reflector from $\mathsf{Anc}(\w)$ to $\w$ restricted to the full subcategory $\prol$. Consequently, in $\w$ involution algebroids are monadic over anchored bundles.
\end{theorem}
\begin{proof}
	Recall the correspondence:
	\[
		\infer{(\hat, \alpha): \wone \to \C \in \mathsf{TangCat}_{lax}}
		{\bar A: \wone \to \C \in \w\cat}
	\]
	Then, if:
	\[
		\wone^* \to \prol \to \wone \to \C	
	\]
	determines an anchored bundle $(\pi:A \to M, \xi, \lambda, \anc)$ whose $V$-coprolongation is $\hat A.V$, so that $\hat A$ is the nerve of an involution algebroid by \Cref{cor:the-prolongation-description}.
\end{proof}
Now, recall that the basic definition of an involution algebroid only really requires prolongations for algebras of width three or less, $T_{i}.T_j.T_k$ so we can use truncation to get the following:
\begin{corollary}
	The category of involution algebroids in a tangent category $\C$ is exactly the pullback:
	\begin{equation}\label{eq:prol3}
		\input{TikzDrawings/Ch5/prol3.tikz}
	\end{equation}
	using the truncated categories from Definition \ref{def:prol-cat} and Definition \ref{def:truncated-wone}
\end{corollary}
In particular, this means that we can write the category of Lie algebroids as a pullback in $\w$-cat:
\begin{corollary}
	The category of Lie algebroids is the pullback in $\w\mathsf{Cat}$:
	\[\input{TikzDrawings/Ch5/lie-algd-monadic.tikz}\]
\end{corollary}



\section{The infinitesimal nerve of a groupoid}%
\label{sec:inf-nerve-of-a-gpd}


The Lie functor, discussed in \Cref{sec:Lie_algebroids} and Example \ref{ex:inv-algds}, is often called the \emph{infinitesimal approximation} of a Lie groupoid (\cite{nlab:lie_group}). This section demonstrates how the enriched categorical perspective on Lie algebroids can make this concrete. Recall that Kan's simplicial approximation functor:

\[
	\mathsf{Top} \to \widehat{\Delta}
\]
Is constructed as a \emph{nerve}, so there is a functor that sends $[n] \in \Delta$ to the $n$-simplex:
\[
	K: \Delta \to \mathsf{Top}; [n] \mapsto \{ x \in \R^n | \sum x \le 1 \}
\] 
The simplicial set approximating a topological space $X$ is exactly $N_K(X)$. The infinitesimal approximation of a groupoid then replaces the simplex category that models homotopical data (the category $\Delta$) with the category of Weil algebras that models infinitesimal data ($\wone$). Thus the infinitesimal approximation of a groupoid will be the nerve of an infinitesimal object:
\[
	\partial: \wone \to \mathsf{Gpd}(\w)
\] so that the nerve $N_\partial$ will coincide with the Lie functor from groupoids to algebroids. This infinitesimal object will also equip the category of groupoids with a second tangent structure, similar to that of Lie algebroids.

This section deals with internal groupoids in the cartesian closed, locally presentable category $\w$. We may use the symmetry of theories to treat:
\[
	\mathsf{Gpd}(\w) \cong \mathsf{Mod}(\wone, \mathsf{Gpd}(\s))
\]
Note that the cofree tangent structure on $\mathsf{Gpd}(\s)$ (recall Observation \ref{obs:cofree-tangent-cat}) agrees with the pointwise tangent structure on internal groupoids.
% A groupoid of particular interest is the \emph{arrow groupoid}.
\begin{definition}%
	\label{def:arrow-gpd}
	The arrow groupoid in $\mathsf{Gpd}(\s)$ is the free groupoid over the graph with a single arrow:
	\[
		\bullet \to \bullet
	\]
	The arrow groupoid in $\w$ is the constant functor:
	\[
		\wone \to \mathsf{Gpd}(\s)
	\]
	Write this internal groupoid $I$, and write the full sub-$\w$-category of $\mathsf{Gpd}(\w)$ spanned by product powers $I^n$ as $\mathbb{I}$.
\end{definition}
\begin{lemma}%
	\label{lem:arr-gpd-cub-monoid}
	The arrow groupoid has two commutative monoid structures on it,
	\[
		\input{TikzDrawings/Ch3/Sec8/cub-mon-gen-maps.tikz}
	\]
	where the multiplications correspond to the maps:
	\[\input{TikzDrawings/Ch3/Sec8/connections-gpd.tikz}\]
	and the units are $s,t:1 \to I$. Note that $t$ is a zero\footnote{A zero for a semigroup is an absorbing element, following the convention from Definition \ref{def:inf-object}.} for the $s$ monoid, and vice versa. The inverse map:
	\[
		i: I \to I
	\]
	exchanges these to monoids: $i \o \gamma^s = \gamma^t$.
\end{lemma}
\begin{remark}
	The arrow groupoid is a \emph{symmetric cubical monoid} (see Section 6 of \cite{Grandis2003}), and the reversion operator makes it a cubical monoid with reversion (see Section 9 of \cite{Grandis2003}, and 8.2 of \cite{Mauri2017}). The cubical perspective presents internal groupoids using commuting squares rather than a composition operation.
\end{remark}
It is well known that the category of internal groupoids is cartesian closed in any locally presentable, cartesian closed category $\C$. Density arguments and the arrow groupoid give way to see this:
\begin{proposition}
	The category of internal groupoids in $\w$ is a cartesian monoidal reflective sub-$\w$-category of $\widehat{\mathbb{I}}$, so it is a cartesian closed, locally presentable $\w$-category.
\end{proposition}
\begin{proof}[(Sketch)]
	This seems to be a piece of mathematical folklore - a proof that groupoids embed into cubical sets may be found in \cite{nlab:fundamental_groupoid_of_a_cubical_set_and_the_cubical_nerve_of_a_groupoid}, where the cubical set is induced using the nerve of the functor $\square \to \mathsf{Gpd}$ induced by cubical monoid $I$, then use the fact that groupoids are an exponential ideal of cubical sets, and apply \Cref{cor:dense-ff-result} to get the desired result that $\mathbb{I}$ is dense in $\mathsf{Gpd}$.
\end{proof}
\begin{corollary}
	The category of internal groupoids in any tangent category $\C$ is a full sub-$\w$-category of $[\mathbb{I}, \C]$.
\end{corollary}

The diagram constructing the linear approximation of a reflexive graph $(s,t:G \to M, i:M \to G)$ is equivalent to an equalizer. Observe that the universality of the following two diagrams is equivalent.
\[\input{TikzDrawings/Ch3/Sec9/Lie-diff-as-eq.tikz}\]
<<<<<<< .mine
A similar argument to Proposition \ref{prop:evf-vbun-is-nonsingular} lets this diagram be presented as an equalizer.
=======
were the target map is $\anc = A \hookrightarrow TG \xrightarrow[]{T.t} TM$.
A similar argument to \Cref{prop:evf-vbun-is-nonsingular} lets this diagram be presented as an equalizer.
>>>>>>> .r7303
\[\input{TikzDrawings/Ch3/Sec9/Lie-diff-as-eq-idempotents.tikz}\]
% \begin{definition}
%     Define $\partial$ to be the coequalizer
%     \[\input{TikzDrawings/Ch5/coeq-partial.tikz}\]
%     Define the following maps on $\partial$.
%     \begin{enumerate}[(i)]
%         \item There is a point $0 \to \partial$ induced by:
%         \[\input{TikzDrawings/Ch5/partial0.tikz}\]
%         \item Write pushout powers of $0$ as $\partial(n)$. 
%         \[\input{TikzDrawings/Ch5/delta-coadd.tikz}\]
%         There is a map $\delta: \partial \to \partial(2)$ induced by:
%         \[\input{TikzDrawings/Ch5/delta-coadd2.tikz}\]
%         \item There is a cosemigroup structure $\odot: \partial \x \partial \to \partial$ induced by:
%         \[\input{TikzDrawings/Ch5/cosemi.tikz}\]
%     \end{enumerate}
% \end{definition}
\begin{definition}%
	\label{def:partial-gpd}
	Define $\partial$ and the map $d:D \to \partial$ to be the following coequalizer in $\mathsf{Gpd}(\w)$.
	\[\input{TikzDrawings/Ch3/Sec9/Lie-diff-as-eq-idempotents.tikz}\]
	where the co-anchor is given by:
	\[
		d := D \xrightarrow[]{(id, t)} D\x I \to \partial
	\]	
\end{definition}

\begin{proposition}
	For any tangent category $\C$, the infinitesimal approximation of the groupoid $G$ (if it exists)
	\[\input{TikzDrawings/Ch3/Sec9/Lie-diff-as-eq.tikz}\]
	Is equivalent to the weighted limit:
	\[
		\{\partial, G\};\hspace{0.25cm} 	\w \xleftarrow[]{\partial} \mathbb{I} \xrightarrow[]{G} \C
	\]
\end{proposition}
\begin{proof}
	Note that by the definition of a weighed limit, for every object $C$ in $\C$
	\[
		\C(C, \{\partial, G\}) \cong [\mathbb{I}, \w](\partial -, \C(C, G-))
	\]
	By the continuity of $ [\mathbb{I}, \w](\partial -, x):\C^{op} \to \w$, it follows that we have the following equalizer diagram for every object $C \in \C_0$:
	\[\input{TikzDrawings/Ch3/Sec9/Lie-diff-as-eq-idempotents.tikz}\]
	which is equivalent to asking that $\{\partial, G\}$ be the equalizer
	\[\input{TikzDrawings/Ch3/Sec9/Lie-diff-as-eq-2.tikz}\]
\end{proof}
\begin{remark}
	The same coequalizer $\partial$ can be constructed in the category of reflexive graphs to exhibit the infinitesimal approximation of a reflexive graph as a weighted colimits.
\end{remark}



\begin{proposition}%
	\label{prop:coeq-of-semigroup-w-z}
	The groupoid $\partial$ in $\mathsf{Gpd}(\w)$ is the coequalizer in the category of semigroups with zeros.
\end{proposition}
\begin{proof}
	First, observe that $(-)\x (=)$ is cocontinuous in each variable, so $\partial \x \partial$ is a double coequalizer - use this to induce a multiplication $\boxdot$.
	\[\input{TikzDrawings/Ch5/induce-obox.tikz}\]
	Where $\tau$ is the natural transformation: \[((\pi_0\o \pi_0, \pi_1 \o \pi_0),(\pi_0\o\pi_1, \pi_1 \o\pi_1))\]
	There is a map:
	\[
		0^\partial:= 1 \xrightarrow[]{(0,s)} D \x I \to \partial	
	\]
	that acts as a zero for the semigroup. 
	The co-continuity of $(-)\x (=)$ in each variable also guarantess that for any semigroup-with-a-zero map:
	\[
		f: D \x I \to X, \hspace{0.15cm}f \o (D \x e^-) = f \o (e \x I)
	\]
	The induced map $f': \partial \to X$ will preserve the multiplication and zero (where the zero is induced by $(0, s): 1 \to D \x I$).
\end{proof}
\begin{corollary}%
	\label{cor:boxdot-coeq}
	The following diagram:
	\[
		\input{TikzDrawings/Ch5/boxdot-coeq.tikz}
	\]
	is a coequalizer.
\end{corollary}
\begin{proof}
	This follows by the commutativity of colimits. The following two diagrams are coequalizers:
	\[\input{TikzDrawings/Ch5/coeqs-mult.tikz}\]
	where $G.2$ is the object of commuting squares, $G_2 \ts{m}{m} G_2$.
	The first couniversality condition is a consequence of the couniversality of $\odot$.
	For the second one, consider the diagram:
	\[\input{TikzDrawings/Ch5/eq-gpd-univ.tikz}\]
	The two equalizer maps send a square to:
	\[\input{TikzDrawings/Ch5/G-univ-maps.tikz}\]
	That is,
	\[
		((v,t), (u,w)): G_2 \ts{m}{m} G_2 \mapsto ((id,u),(u,id)), ((v,id),(id,v))
	\]
	So for a square to $((v,t), (u,w))$ be equalized by these two maps, it follows that:
	\[
		v = id, u = id
	\]
	so the square must be of the form $((id,t),(id,w)):G_2 \ts{m}{m} G_2$, thus $t = w$, and the square is $G^{\square +}(t)$.
\end{proof}

\begin{lemma}%
	\label{lem:co-anchored-bundle-gpd}
	The tuple:
	\[
		(y: D \x \partial \xrightarrow[]{d \x \partial} \partial \x \partial \xrightarrow[]{\boxdot}\partial, 0: 1 \to \partial, !:\partial \to 1, d:D \to \partial)
	\]
	is a co-anchored bundle under $1$, where
	\[
		y: D \x \partial \xrightarrow[]{d \x \partial} \partial \x \partial \xrightarrow[]{\boxdot} \partial
	\]
\end{lemma}

\begin{proposition}
	For every Weil algebra $V$, there is an isomorphism:
	\[
		L_V \cong \partial_V
	\]

	Where$L_V$ is the $V$-prolongation of the co-anchored bundle in Lemma \ref{lem:co-anchored-bundle-gpd}.
\end{proposition}

\begin{proof}
	Without any loss in generality, it is sufficient to prove this holds for $L_{n} = L(W_n)$ and $n\cdot \partial$. The proof follows by induction, first note that $L = \partial$ by definition.

	For $L_2$ and $\partial \x \partial$, first note there is the injection:
	\[\input{TikzDrawings/Ch5/induce-map-from-coprol.tikz}\]
	Note that for any $G$, a map $X: \partial \x \partial \to G$ corresponds to a commuting square in $T^2G$ of the form:
	\[\input{TikzDrawings/Ch5/comm-square-T2G.tikz}\]
	so that $T.e \o v = id, e.T \o u = id$.
	Note that $u = (e.T \o v)^{-1};(T.e \o u);v$, and that precomposition with the uniquely induces map determine a $(\bar{u},v):X \to G^{L(2)}$, where
	\[ T.0 \o \bar{u} = u\]
	Observe that any pair $(\bar{u}, v):X \to  G^{L(2)}$ determines a square:
	\[
		\input{TikzDrawings/Ch5/inverse-of-prol.tikz}
	\]
	where $T.e \o v = id$, and $T.e \o \bar{u} = id$.
	Note that $T.0 \o T.p \o T.0 \o \bar{u} = T.0 \o \bar{u}$, and that the bottom horn is $u = (e.T \o v)^{-1};(T.0 \o \bar{u});v$, now check:
	\begin{align*}
		T.e \o u
		% &= T.e \o \((e.T \o v)^{-1};(T.0 \o \bar{u});v \) \\
		 & = (T.e \o e.T \o v)^{-1};(T.e \o T.0 \o \bar{u});(T.e \o v) \\
		 & = id; T.0 \o \bar{u}; T.e \o v = T.0 \o \bar{u}
	\end{align*}
	and
	\begin{align*}
		e.T \o u
		 & = e.T \o (e.T \o v)^{-1};(T.0 \o \bar{u});v                 \\
		 & = (e.T \o e.T \o v)^{-1};(e.T \o T.0 \o \bar{u});(e.T \o v) \\
		 & = (e.T \o v)^{-1};id;(e.T \o v) = id
	\end{align*}
	Thus determining a map $X \to G^{\partial \x \partial}$.
	The two maps are inverse to each other, giving an isomorphism.

	% For the inductive case, use the zig-zag presentation of $G^{L(n+2)}$ to see the following isomorphism holds:
	% \[
	%     \input{TikzDrawings/Ch5/inductive-step.tikz}
	% \]
	% Thus, $L(n) = D(n)$.

	For the inductive case, look at the prolongations of anchored bundles and recall that:
	\[
		\prol(UV,A) \boxtimes_M \prol(Z,A)  =
		\prol(UV,A) \boxtimes_{\prol(U,A)} \prol(UZ,A)
	\]
	Where you treat $\prol(UV,A), \prol(UZ,A)$ as spans over $\prol(U,A)$, so that:
	\begin{gather*}
		\prol(U,A) \xleftarrow[]{id \boxtimes \pi^V} \prol(UV,A) \xrightarrow[]{anc^U \boxtimes \prol(V,A)} T^U.\prol(V,A)\\
		\prol(U,A) \xleftarrow[]{id \boxtimes \pi^Z} \prol(UZ,A) \xrightarrow[]{anc^U \boxtimes \prol(Z,A)} T^U.\prol(Z,A)
	\end{gather*}
	And observe that their span composition is:
	\[
		\input{TikzDrawings/Ch5/pullback-uvz.tikz}
	\]
	Now, assume that the hypothesis holds for any two of $U, V, Z \in \wone$ and use the co-continuity of $X \x (-)$ in a cartesian closed category.
	\begin{align*}
		L_{UVZ} & = L_{UV} \boxplus_U L_{UZ}
		% \\
		% &= (\partial(U) \x \partial(V)) \po_{(id)}{\pi_0} (D(V) \x \partial(U) \x \partial(Z)) \\
		% &= \partial(U) \x (\partial(U) \po_{}{} \partial(Z)) \\
		% &= \partial(V) \x \partial(U)\x \partial(Z)
	\end{align*}
	So it now suffices to prove that the diagram:
	\[\input{TikzDrawings/Ch5/partial-u-po.tikz}\]
	is a pushout - but by the inductive hypothesis,
	\[\input{TikzDrawings/Ch5/partial-no-u-po.tikz}\]
	so the result follows by the cocontinuity of $\partial_U \x (-)$.
	% (where you use the hypothesis for the co-anchored bundle $\boxplus_U$ )
\end{proof}
\begin{corollary}%
	\label{cor:rewrite-boxdot}
	Note that, by construction, the $\hat{y}:L_{WW} \to L$ map is isomorphic to the $\boxdot$ multiplication.
	\[
		\hat{y}: L_{WW} \cong \partial \x \partial \xrightarrow[]{\boxtimes} \partial
	\]
\end{corollary}

\begin{theorem}%
	\label{thm:inf-gpd}
	The object $\partial$ determines a monoidal, transverse-colimit-preserving $\w$-functor:
	\[
		\partial: \wone \to \mathsf{Gpd}(\w)
	\]
	with a monoidal natural transformation $d:\partial \Rightarrow D$.
\end{theorem}
\begin{proof}
	First, check that $(\partial, \boxtimes, 0, !, \delta)$ is an infinitesimal object Definition \ref{def:inf-object}.
	\begin{enumerate}[{[{I}O.1]}]
		\item Pushout powers of $0:1 \to \partial$ exist as $\mathsf{Gpd}(\w)$ is cocomplete.
		\item The commutative-semigroup-with-a-zero axiom follows by Proposition \ref{prop:coeq-of-semigroup-w-z}
		\item The additivity follows from Corollary \ref{cor:rewrite-boxdot}
		\item The couniversality axiom follows from the couniversality of the underlying coanchored bundle and Corollary \ref{cor:rewrite-boxdot}.
	\end{enumerate}
	Note that $d: D \to \partial$ commutes will all of the structure morphisms, so it induces a monoidal natural transformation $D \Rightarrow \partial$, exhibiting $\partial$ as an enriched functor.
\end{proof}


\begin{definition}
	By Theorem \ref{thm:inf-gpd}, there is a $\w$-functor:
	\[
		\partial: \wone^{op} \to \mathsf{Gpd}(\w)
	\]
	The nerve of $\partial$ is the \emph{infinitesimal nerve} functor (the nerve of an infinitesimal object).
\end{definition}
\begin{theorem}
	The infinitesimal nerve of $\partial: \wone \to \mathsf{Gpd}$ lands in the category of involution algebroids.
\end{theorem}
\begin{proof}
	Observe that the underlying co-anchored bundle structure on $\partial$ induces a functor:
	\[
		L: \prol \to \mathsf{Gpd}(\w)
	\]
	so that $N_L$ lands in the $\prol$-nerves for $\mathsf{Anc}(\w)$. Therefore, the following diagram commutes:
	\[\input{TikzDrawings/Ch5/inf-nerve-wonky.tikz}\]
\end{proof}
\begin{observation}%
	\label{obs:derivative-weighted-limit}
	If all limits weighted by $W:\a \to \w$ exist in $\C$, then this gives a functor:
	\[
		[\a, \C ] \xrightarrow[]{\{W,-\}} \C; F \mapsto \{ W, F\}
	\]
	which may also be regarded as a functor:
	\[
		\{-,-\}: [\a, \w] \x [\a, \C] \to \C 	
	\]
	Now, regard the infinitesimal object $\partial$ as the weight:
	\[
		\partial: \wone \x \square^{op} \to \w; (V, [n]) \mapsto \partial_V([n])
	\]
	And a groupoid $\g$ as a strict tangent functor:
	\[
		G:\wone \x \square^{op} \to \C	
	\]
	Then the Lie functor is equivalently given as the weighted limit:
	\[
		`G^\partial: \wone^{op} \xrightarrow[]{\widehat{(\partial, G)}} 
		[\square^{op}, \w] \x [\square^{op}, \C] \xrightarrow[]{\{-,-\}} \C
	\]	
	% (regarding $\wone \x \square^{op}$ as the free tangent category over $\square^{op}$).
	% Then for any groupoid $G: \wone \x \square^{op} \to \C$, the Lie derivative is computed as the partial weighted-limit 
	% \[
	% 	\{\partial_{\wone}, -\}: \mathsf{Gpd}(\C) \to \mathsf{Inv}(\C)
	% \]
\end{observation}

Now that the Lie derivative in $\w$ has been characterized as the nerve of 
\[
	\partial: \wone \to \w
\]	
This has put the Lie functor into a nerve/realization context (recall \Cref{def:nerve}).
\begin{definition}
	The \emph{Lie realization} is the left Kan extension:
	\[
		|-|_\partial = Lan_\partial: \mathsf{Inv}(\w) \to \mathsf{Gpd}(\w)	
	\]
\end{definition}

This functor is well behaved - first see that it preserved products:
\begin{lemma}
	The realization functor preserves products.
\end{lemma}
\begin{proof}
	Product-preservation is a consequence of $|-|_\partial$ being the left Kan extension of a cartesian functor along a cartesian functor.
	Note that this means $\int^v\partial(v) = 1$.
\end{proof}
Next, we see that the realization of an involution algebroid has the same base space.

\begin{lemma}\label{lem:base-of-groupoid}
	The base space of the groupoid $\partial$ is $D^v$.
\end{lemma}
\begin{proof}
	When constructing the colimit of groupoids, the colimit's base space is the ordinary colimit for the diagram of the base spaces. The reflector from simplicial objects to groupoids preserves products, so it suffices to check that the base space of $\partial(n)$ is $D(n)$.

	The base space of $I$ is $1+1$, as:
	\[
		I(0) = \widehat{\square}(1,I) \cong \square(0,I) = 1 + 1
	\]
	and the map $e^-_0$ is given by $\delta^- \o !$.
	$D$ is a discrete cubical object, so the base space is $D \x 1$.
	Thus the coequalizer defining $\partial$ is:
	\[\input{TikzDrawings/Ch5/coeq-def-partial.tikz}\]
	A map $\gamma: D + D \to M$ is a pair of maps $\gamma_0, \gamma_1: D \to M$.
	We can see that $\gamma_0, \gamma_1$ agree at $0$ (they are both $\gamma_0(0)$), and $\gamma(0)$ is a constant tangent vector. It follows then, that $\gamma_1 \o (id | id) = \gamma$.
\end{proof}

Now, recall the co-Yoneda lemma, for any $\vv$-presheaf $A: \C^{op} \to \vv$
\[
	F(C) = \int^{C' \in \C} \C(C,C') \ox F(C')
\]
In particular, for an involution algebroid in $\w$ (or any $\w$-presheaf on $\wone^{op}$)
\[
	A(U) = \int^{V \in \wone} \wone^{op}(U,V) \x A(V) = \int^{V \in \wone} \wone(V,U) \x A(V)
\]
\begin{lemma}\label{lem:as-a-presheaf}
	For any involution algebroid $A$:
	\[ A(R) = \int^{V \in \wone} A(V) \x D^V \]
\end{lemma}
\begin{proof}
	Use the tangent structure on $\wone$ to regard it as a $\w$-enriched category:
	\begin{gather*}
		D^V = \yon(V) = \wone(V,-) = (U \mapsto \wone(V, U))  \\= (U \mapsto \wone(V, U\ox R)) = \wone(V,R)
	\end{gather*}
	The following computation gives the result:
	\[
		A(R) = \int^{V} \wone(V,R) \x A(V) = \int^{V} D^V \x A(V)
	\]
\end{proof}
We can now see that the base space of an involution algebroid and its realization are isomorphic.

\begin{proposition}\label{prop:lie-int-first-part}
	Let $A$ be an involution algebroid in $\w$. Then $|A|([0]) = A(R)$.
\end{proposition}
\begin{proof}
	Use the Yoneda lemma, and that $\yon[0] = 1$ is a small projective so $\mathsf{Gpd}(1,-)$ is $\w$-cocontinuous, then apply Lemma \ref{lem:base-of-groupoid} and Lemma \ref{lem:as-a-presheaf}
	\begin{align*}
		|A|([0]) & = \mathsf{Gpd}(1, |A|)                                                   \\
		         & = \mathsf{Gpd}\left(1, \int^{v \in \wone} A(v)\bullet \partial v \right) \\
		         & = \int^{v} A(v)\x \mathsf{Gpd}(1,  \partial v )                          \\
		         & = \int^{v}  A(v)\x D^v = A(R)
	\end{align*}
\end{proof}

Thus, as a final result, we have achieved an adjunction between the category of involution algebroids and groupoids in $\w$, that is product-preserving and stable over the base spaces.
\begin{theorem}[The Lie Realization]%
	\label{thm:lie-realization}
	There is an adjunction between the category of involution algebroids and groupoids internal to $\w$, where each functor preserves products and the base spaces.
	\[% https://q.uiver.app/?q=WzAsMixbMCwwLCJcXG1hdGhzZntHcGR9KFxcdykiXSxbMSwwLCJcXG1hdGhzZntJbnZ9KFxcdykiXSxbMCwxLCJOX1xccGFydGlhbCIsMCx7ImN1cnZlIjotMn1dLFsxLDAsInwtfF9cXHBhcnRpYWwiLDAseyJjdXJ2ZSI6LTJ9XSxbMiwzLCIiLDAseyJsZXZlbCI6MSwic3R5bGUiOnsibmFtZSI6ImFkanVuY3Rpb24ifX1dXQ==
	\begin{tikzcd}
		{\mathsf{Gpd}(\w)} & {\mathsf{Inv}(\w)}
		\arrow[""{name=0, anchor=center, inner sep=0}, "{N_\partial}", curve={height=-12pt}, from=1-1, to=1-2]
		\arrow[""{name=1, anchor=center, inner sep=0}, "{|-|_\partial}", curve={height=-12pt}, from=1-2, to=1-1]
		\arrow["\dashv"{anchor=center, rotate=-90}, draw=none, from=0, to=1]
	\end{tikzcd}\]
\end{theorem}



==> Chapters/Ch5-InfNerve-orig.tex <==
% \documentclass[main.tex]{subfiles}

% \begin{document}

\chapter{The infinitesimal nerve and its realization}%
\label{ch:inf-nerve-and-realization}

This chapter makes use of \emph{enriched nerve} constructions, transferring a classical construction in categorical topology to categorical Lie theory. Recall simplicial localization functor of \cite{Kan1958}, which sends a topological space to $X$ to the simplicial set:
\[
    N_\Delta(X): \Delta^{op} \to \s; [n] \mapsto \mathsf{Top}(\Delta_n, X)
\]
where $\Delta_n$ is the subset of $\R^n$ spanned by:
\[
    \{
        (x_1, \dots, x_n) \in \R^n | \sum x_i \le 1
    \}    
\]
That is, the geometric $n$-simplex. The simplicial set $N_\partial(X)$ can be considered the simplicial approximation of the topological space $X$.
Kan showed that the \emph{topological realization} functor, induced by the left Kan extension:
\[\input{TikzDrawings/Ch5/top-real.tikz}\]
Kan's construction induces an adjunction between simplicial sets and topological spaces, and is essential in relating the homotopy structure on simplicial sets to that of topological spaces.
Our goal, then, is to construct an ``infinitesimal'' version of this story on the category of groupoids in a (suffiently well-behaved) tangent category, so that we induce an adjunction:
\[\input{TikzDrawings/Ch5/lie-adj.tikz}\]
This will similarly construct an adjoint pair between the Lie functor:
\[
    \mathsf{Lie}: \mathsf{Gpd} \to \mathsf{Inv}  
\]
and a \emph{Lie realization} functor, that associates a groupoid to an involution algebroid.


\section{Tangent categories via enrichment}%
\label{sec:tang-cats-enrichment}

In this section demonstrates how tangent categories fit inside the framework of enriched categories.  This was first demonstrated in \cite{Garner2018}, building on the actegory perspective on tangent categories introduced in \cite{Leung2017} and a result relating monoidal actions and enrichment from \cite{Wood1978}. This is mostly expository, however we make time to consider the differential objects in the enriching tangent category, the category of Weil spaces.


Weil spaces are closely related to the \emph{Weil topos}, introduced by Dubuc in his original study of models of synthetic differential geometry \cite{Dubuc1981}. The Weil topos is not a well-adapted model of synthetic differential geometry, and was mostly treated as a toy model, although a deeper study of the topos may be found in \cite{Bertram2014}. Recall that the category $\wone$ is the free tangent category over a single object. The category of Weil spaces may be identified as the \emph{cofree} tangent category over $\s$, which is $\mathsf{Mod}(\wone, \s)$ from Observation \ref{obs:cofree-tangent-cat}. Call this the category of \emph{Weil spaces}, and write it $\w$. Just as a simplicial set $S: \delta \to \s$ can be thought of as a gadget recording homotopical data, a Weil space is a gadget recording \emph{infinitesimal} data.

\begin{definition}
	A \emph{Weil space} is a functor $\wone \to \s$ that preserves transverse limits - that is, the $\ox$-closure of the set of limits:
    \[
        \left\{
            \input{TikzDrawings/Ch5/wone-pb.tikz}
            ,
            \input{TikzDrawings/Ch5/wone-univ-lift.tikz}
            ,
            \input{TikzDrawings/Ch5/wone-id.tikz}
        \right\}
    \]  
	A morphism of Weil spaces is a natural transformation. The category of Weil spaces is written $\w$.
\end{definition}
\begin{example}
	~\begin{enumerate}[(i)]
		\item Every commutative monoid may be regarded as a Weil space in a canonical way.
		Observe that for every $V \in \wone$ and commutative monoid $M$, there is a free $V$-module structure on $M$ given by $|V| \ox_{\mathsf{CMon}} M$.
		The underlying commutative monoid of $V$ is exactly $\N^{\mathsf{\dim V}}$, so that:
		\[
			V \bullet M \cong \oplus^{\dim V} M 	
		\]
		The microlinearity of $V \mapsto |V| \ox M$ follows from basic properties of finite biproducts.
        \item Following (i), any tangent category $\C$ that is \emph{concrete} - it admits a faithful functor $U_\s: \C \to \s$ - will have a natural functor into tangent sets (copresheaves on $\wone$).
        Every object $A$ will have an underlying tangent set $V \mapsto U_{\s}(T^V(A))$, and whenever $U_\s$ preserves connected limits (such as the forgetful functor from commutative monoids to sets), each of the underlying tangent sets will be a propert Weil space.
		\item Consider a symmetric monoidal category with an infinitesimal object, which by \Cref{cor:rewrite-rep-functor} is a transverse colimit preserving symmetric monoidal functor $D:\wone \to \C$. Then for every object, the nerve (\Cref{def:nerve}) $N_D(X): \C(D-,X):\wone \to \s$ is a Weil space. 
		\item For any pair of objects $A,B$ in a tangent category, $\C(A,T^{(-)}B):\wone \to \s$ is a Weil space by the continuity of $\C(B,-):\C \to \s$.
	\end{enumerate}
\end{example}
Unlike the category of simplicial sets, the category of Weil spaces is not a topos due to the restriction to transverse-limit-preserving functors.
The category of Weil spaces does, however, inherit some nice properties from the topos of copresheaves on $\wone$ by applying results from \cref{sec:enriched-nerve-constructions}.
\begin{proposition}[\cite{Garner2018}]
	The category of Weil spaces is a cartesian-monoidal reflective subcategory of $[\wone,\s]$.
\end{proposition}
\begin{corollary}
	The category of Weil spaces is:
	\begin{enumerate}[(i)]
		\item A cartesian closed category.
		\item Locally finitely presentable as a cartesian monoidal category (as in \cref{def:v-lfp}).
		\item A representable tangent category, using $\yon: \wone^{op} \to \w \hookrightarrow [\wone,\s]$.
	\end{enumerate}
\end{corollary}
The cofree tangent structure on $\w$ is given by precomposition, that is:
\[
	T^U.M.(V) = M.(U \ox V) = M.T^U.V
\]
This tangent coincides with the representable tangent structure induced by the Yoneda embedding, which can be seen using a simple application of the Yoneda lemma. The proof is a simple application of the Yoneda lemma. Observe:
\[
    [D,M](V) \cong [\wone,\s](D \x \yon(V), M) \cong [\wone, \s](\yon(T.V)), M) \cong M(T.V)
\]
where $D \x \yon(V) = \yon(T.V)$ as the tensor product in $\wone$ is cocartesian.

% Thus, we set the following piece of notation/terminology:
% \begin{notation}
% 	For a structure in a tangent category (e.g. a differential object, involution algebroid, etc), we call a model of $X$ in $\w$ a tangent $X$.
% \end{notation}

% % \paragraph{The enrichment of a tangent category in $\w$}%
% % \label{sub:enrichment-of-tang-cat}
% The basic idea in enriched category theory is that the definition of a category involves very little about the category of sets.
% Thus, we can define for any monoidal $\vv^\ox$ the notion of a $\vv$-category.


In general, any actegory over a monoidal $\C$ will give rise to $[\C,\s]$-enriched category, using the tensor structure induced by Day convolution, was proved by \cite{Wood1978}, that tangent categories are certain class of enriched category is a consequence of that result when combined with Leung's actegory result.
% We will only look at the result for tangent categories.
\begin{proposition}
	Every tangent structure $(\C, \T)$ equips $\C$ with an enrichment in Weil spaces.
\end{proposition}
\begin{proof}
	The presheaf is constructed:
	\[
		\underline{\C}(A,B) = \C(A, T^{}B): \wone \to \s 
	\]
	The functor $\C(A,-)$ is continuous and $T^{-}B$ is a microlinear complex, so this is a Weil space. The composition map is constructed as:
	\input{TikzDrawings/Ch5/enrichment-in-W-comp.tikz}
	which is natural in $U,V$.
\end{proof}
The following coherence on powers was defined by \cite{LucyshynWright2016}.
\begin{definition}
	Let $\j \hookleftarrow \vv$ be a full monoidal subcategory of $\vv$. A $\vv$-category $\C$ has \emph{coherently chosen powers} by $\j$ if there is a choice of $\j$-powers $(-)^J$ so that:
	\[
		(C^J)^K \cong C^{J \ox K}
	\]
	and coherence chosen copowers whenever there is a choice of $\j$-copowers so that:
	\[
		K \bullet (J \bullet C) \cong (K \ox J) \bullet C	
	\]
	The sub-2-category of $\vv$-categories equipped with coherently chosen powers and copowers are $\vv\cat^\j$ and $\vv\cat_\j$, respectively.
\end{definition}

Now, returning to the specific enrichment in $\w$, remember that the hom-object between $A,B$ is given by:
\[	
	V \mapsto \C(A,T^V B)
\]
For a representable functor $\yon U$, use the fact that the representable tangent structure induced by $\yon$ coincides with the cofree tangent structure, and find:
\[
	\w(\yon U, V \mapsto \C(A, T^VB)) \cong V \mapsto \C(A, T^V.T^U(B))
\]
Then, a tangent category (and any actegory, really) does not simply have an enrichment in $\w$, it also has coherently chosen powers by representables. In fact, $\w$-categories with coherently chosen powers by representables are \emph{exactly} the $\w$ categories that are induced by a tangent structure. Thus we have the following:
\begin{proposition}[\cite{Garner2018}]
	A tangent category is exactly an $\w$-category with coherently chosen powers by representables.
\end{proposition}
Now the original notions of (lax, strong, strict) tangent functors can be defined as $\w$-functors between $\w$-categories with coherently chosen powers, where the lax/strong/strict adjective now relates to the preservation of the coherently chosen powers.
\begin{theorem}[\cite{Garner2018}]
	We have the following equivalences of 2-categories.
	\begin{enumerate}[(i)]
		\item The 2-category of $\w$-categories with coherently chosen powers and $\mathsf{TangCat}_{\mathsf{Lax}}$
		\item The 2-category of $\w$-categories with coherently chosen powers and power-preserving $\w$ functors  and $\mathsf{TangCat}_{\mathsf{Strong}}$
		\item The 2-category of $\w$-categories with coherently chosen powers and chosen-power-preserving $\w$ functors $\mathsf{TangCat}_{\mathsf{Strict}}$
	\end{enumerate}
\end{theorem}
Now, the Yoneda lemma applies of $\w$-categories. So a tangent category may be embedded into its $\w$-category of tangent presheaves:
\[
	F: \C^{op} \to \w 
\]
The powers by representables are computed pointwise, and so they inherit the coherently choice. Thus the following holds:
\begin{corollary}
	Every tangent category embeds into a representable tangent category
	\[
		\C \hookrightarrow [\C^{op},\w] = \widehat\C
	\]
\end{corollary}

% \paragraph{Differential objects and commutative monoids}
% As an application of the enriched perspective of tangent categories, consider the category differential objects in $\w$.
% We find that the category of differential objects is isomorphic to the replete image of $\mathsf{CMon}$ into the category of Weil spaces. 
% \begin{lemma}\label{lem:cmon-tang-inclusion}
% 	There is a cartesian $\w$-inclusion $d:\mathsf{CMon} \hookrightarrow \w$, where $\mathsf{CMon}$ is regarded as a tangent category using the biproduct structure.
% \end{lemma}
% \begin{proof}
% 	Note that because $\mathsf{CMon}$ is a cartesian tangent category, we have powers by representables given by:
% 	\[
% 		A^{W^{n_1} \dots W^{n_k}} = T_{n_1}\circ\dots\circ T_{n_k}(A)
% 	\]
% 	thus we can send $A$ to the presheaf $V \mapsto A^V$.
% \end{proof}
% \begin{remark}
%     It is worth noting that every category with biproducts has this tangent structure, and recalling that product-preserving tangent functors preserve differential objects. Since a cartesian differential category is equivalently a cartesian tangent category with a coherent choice of differential objects, this leads to the idea that ``a CDC is a CLAC in $\w\cat$'' - that is, a cartesian differential category is exactly a $\w$-category $\C$ where there is a category with biproducts $\C^+$ (regarded as a tangent category) and a bijective-on-objects $\w$-functor:
%     \[
%       \C^+ \hookrightarrow \C   
%     \] that creates products and powers by representable functors - this is a straightforward generalization of \Cref*{prop:clac-defs} from cartesian left addtive categories to cartesian differential categories.
% \end{remark}

% \begin{lemma}\label{lem:diff-ob-w-determines-cmon}
% 	A differential object in $\w$ uniquely determines a commutative monoid in $\s$.
% \end{lemma}
% \begin{proof}
% 	First, note that by the symmetry of theories, a commutative monoid in $\w$ is a model of Weil algebras and transverse limits into commutative monoids. This means that for a differential object $(A,+',0')$, we have a commutative monoid
% 	\[
% 		A(R) \times A(R) \xrightarrow{+'_R} A(R) \hspace{0.5cm} 0': 1 \to A(R)
% 	\]
% 	The coherence that $TA \cong A \times A$, and that $+_A$ may be rewritten as $+'$, means that 
% 	\[
%     \input{TikzDrawings/Ch5/wsp-cmon-plus.tikz}
% 	\]
% 	Thus we can see that $A(W^{n_1} \dots W^{n_k}) \cong A(R)^{\prod (n_i + 1)}$. 
% 	Therefore $A$ is determined, up to a unique isomorphism, by the inclusion $(A(R),+'_R,0'_R)$ from $\mathsf{CMon}$ into $\w$.
% \end{proof}
% \Cref{lem:cmon-tang-inclusion} and \cref{lem:diff-ob-w-determines-cmon} yield the following equivalence of categories. 
% \begin{proposition}\label{prop:diff-ob-is-CMon}
% 	The category of differential objects in $\w$ is $\w$-equivalent to the category of commutative monoids.
% \end{proposition}

% We now look at some characterizations of the natural numbers $d(\N)$ in $\w$ - which we will often call $\N$.
% We may associate the ring $\N$ with a certain pullback involving the infinitesimal $D$, and the underlying Weil algebra functor.
% \begin{proposition}\label{prop:ring_properties}
%     Denote the inclusion $I: \mathbf{CMon} \hookrightarrow \w$. The following are equivalent:
%     \begin{enumerate}[(i)]
%         \item $\mathbb{N}$
%         \item The underlying set functor $U:\mathbf{Weil}_1 \to \mathbf{Set}$
%         \item The pullback
%             \input{TikzDrawings/Ch5/N-as-pb.tikz}
%             with $\sigma_A$ induced by $+_D$ and multiplication given by composition.
%     \end{enumerate}
%     Call this universal ring object $R$.
% \end{proposition}
% \begin{proof}
%     We first observe that $\mathcal{U} \cong d(\mathbb{N})$, as $\N$ sends a Weil algebra $W^{n_1} \dots W^{n_k}$ to the underlying set of the commutative monoid $\N^{W^{n_1} \dots W^{n_k}}$.
%     The underlying commutative monoid of $W^{n_1} \dots W^{n_k}$ is 
%     \[ \N^{n_1 + 1} \ox \dots \ox\N^{n_k +1} \cong \N^{\prod n_i + 1} \cong T_{n_1} \dots \circ T_{n_k}\N\]
% 	Thus the isomorphism holds.
    
%     To show $d(\N) \cong [D,D]_0$, first calculate the presheaf $[D,D]$:
%     \begin{align*}
%     [D,D](V)   &\simeq [\yon.T,\yon.T](V) \\
%                &\simeq \mathsf{Nat}(\yon.T \x \yon.T^V,\yon(x^2))\\ 
%                &\simeq \mathsf{Nat}(\yon.T.T^V,\yon.T) \\
%                &\simeq \mathsf{Weil}(T,T.V)
%   \end{align*}
%   Then we may compute the pullback (2) point-wise:
%   \[
%      \input{TikzDrawings/Ch5/two-as-pointwise.tikz}
%   \]
%   First, note that $R(0) = \mathsf{Weil}(x^2,x^2) = \mathbb{N}$ as the only endomorphisms for $\N[x]/x^2$ in $\mathsf{Weil}$ are scalar multiplication $x \mapsto nx$. 
%   $R$ is a differential object by \cref{lem:tang-space-diff-ob}, so by Proposition \ref{lem:diff-ob-w-determines-cmon}, $R(W) \cong \mathbb{N}^W$ and the ring isomorphism $[D,D]_0 \cong I(\mathbb{N})$ is immediate.
% \end{proof}
% \begin{lemma}\label{lem:action_on_T}
%     In a tangent category $\mathbb{C}$, the action of $\mathbb{N}$ on $(p_M, +_m, 0_M)$ coincides with the $ \mathcal{W}$-natural transformations induced by the inclusion \[\N \hookrightarrow [D,D] \to \w\mathbf{nat}(T,T)\]
% \end{lemma} 

% Now, we observe a particularly useful Weil space:
% \begin{definition}
%     Let $E$ be a commutative monoid. The free vector over $E$ is the Weil space $E_0$ where:
%     \[
%         E_0(V) = E^{\dim(V)-1}
%     \]
%     Each $V$ is the fiber of $E(V)$ over $E(\N) \to^{0^V} E(V)$, and the structure transformations are defined accordingly.
% \end{definition}


\section{Enriched nerve constructions}%
\label{sec:enriched-nerve-constructions}

This chapter will be making use of enriched nerve constructions, as developed in \cite{Bourke2019}. 
These constructions will make formal the intuitive notions of the ``Weil nerve'' and the ``Segal conditions for involution algebroids'' developed in \Cref{chap:weil-nerve}. In order to keep this chapter relatively self-contained, this section includes a basic introduction to locally presentable enriched categories, the nerve/realization paradigm, and the notion of a nervous theory.

% \paragraph{A review of locally finitely presentable $\vv$-categories}



% \paragraph{Monads and theories}
The ``nerve'' of an internal category and involution algebroid were discussed in \Cref{sec:nerve-of-a-category,sub:microlinear-nerve-of-an-involution-algebroid}, although the notion of a nerve or Segal condition was not made precise. This section concludes by giving the formal theory of nerves/Segal-condition paradigm from  \cite{Berger2012,Bourke2019}, and the the nerve/realization paradigm in \cite{loregian2015}.

\begin{definition}%
    \label{def:nerve}
    The \emph{nerve} of a $\vv$-functor $K: \a \to \C$ is the functor
    \[
        N_K: \C \to \widehat{\a}; \hspace{0.5cm} C \mapsto \C(K-, C)    
    \]
    (where $\widehat{A}$ is the $\vv$-category of $\vv$-presheaves on small $\vv$-category $A$).
    Whenever $\C$ is cocomplete, the nerve has a left adjoint called the \emph{realization}, computed by the left Kan extension/coend:
    \[
        \input{TikzDrawings/Ch5/realization.tikz}
        \hspace{0.5cm}
        |C|_K := \int^A \C(KA, C) \cdot KA
    \]
    A \emph{nerve/realization context} is $\vv$-functor $K:\a \to \C$ from a small $A$ to a cocomplete $\C$.
\end{definition}
% We can see that the nerve itself may be represented as a left Kan extension:
% \begin{lemma}
The nerve functor itself is equivalently the left Kan extension of $K$ along $\yon$:
\[\input{TikzDrawings/Ch5/nerve-is-lany.tikz}\]
For a proof see \cite{loregian2015}. This gives the unusual property that the nerve/realization adjunction is of the form:
\[
    Lan_{\yon}K \vvdash Lan_K\yon
\]

\begin{example}
    ~\begin{enumerate}[(i)]
        \item Recall the original construction of the simplicial nerve of a topological space $X$, where $X_n = \mathsf{Top}(\Delta_n,X)$.
        This is exactly the nerve of the functor $\bar{\Delta} \to \mathsf{Top}$ that sends $n$ to the $n$-simplex:
        \[
            \{
                x \in \R^n | \sum x_i = 1
            \}
        \]
        \item The theory of locally finitely presentable categories gives a useful class of examples.
        Because we may represent a locally presentable $\C$ as $\mathsf{Lex}(\C_{fp}^{op}, \vv)$ (whenever $\vv$ itself is locally presentable as a closed category), we can see that the nerve of $\C_{fp} \hookrightarrow \C$ is a fully faithful functor, and the realization is the reflection from presheaves on $\C_{fp}$ to models.
    \end{enumerate}
\end{example}

The situation where the nerve of $K$ is fully-faithful particularly important. Kelly called these subcategories \emph{dense}, by metaphor with the notion of density found in Hausdorff spaces. A dense subcategory models the same situation, except we replace ``continuous functions'' with ``cocontinuous functors''. That is to say, a functor $K:\a \to \c$ into a cocomplete $\c$ is \textit{dense} whenever each object $C \in \c_0$ is canonically written as a coend:
\[
	\int^A \C(KA, C)\cdot KA
\]
so that a cocontinuous functor $F:\c \to \d$ is determined by $F.K$.
The general definition of density does not require a cocomplete category.
\begin{definition}
	A functor $K: \a \to \C$ is \textit{dense} whenever one of the following conditions holds
	\begin{itemize}
		\item The identity functor $id:\C \to \C$ is the left Kan extension of $K$ along itself, so: $Lan_K K = id$.
		\item Every object is given as the weighted colimit $C = N_K(C) \star K$.
		\item The nerve of $K$ is fully faithful.
	\end{itemize}
\end{definition}
Dense functors are poorly behaved under composition, but there is a useful cancellativity results from Chapter 5.2 of \cite{Kelly2005}.
\begin{proposition}
    Consider a diagram of $\vv$-categories
    \[\input{TikzDrawings/Ch5/lan-result.tikz}\]
    where $\alpha$ is a natural isomorphism, and $K$ is dense. 
    If this diagram exhibits $(\alpha, J)$ as the left Kan extension of $K$ along $F$, then $J$ is dense.
\end{proposition}
\begin{corollary}%
    \label{cor:dense-ff-result}
    If $K$ is dense, $F$ is fully faithful, and  $J.F = K$, then $F$ is a dense subcategory.s
\end{corollary}
Generally speaking, we will often refer to dense \textit{subcategories} rather than dense \textit{functors}. Through a naive application of the (bo,ff)-factorization system on $\vv$-categories, every dense functor induces a dense subcategory, as $K$ factors as
\[
    K = \a \xrightarrow[]{K'} \mathsf{im}(K) \hookrightarrow \C
\]
so the inclusion of $\mathsf{im}(K)$ into $\C$ is dense.
% \begin{proposition}
% 	Let $K:A \to \c$ be a dense functor. Then the full subcategory $im(K)$ is a dense subcategory.
% \end{proposition}
% \begin{proof}
% 	Use \cref{cor:dense-ff-result}.
% \end{proof}
% \begin{example}
% 	Consider the category of transverse-limit preserving copresheaves of $\wone$ algebras $\w = \mathsf{Mod}(\wone, \s)$, the category of Weil spaces. We have the following dense subcategories:
% 	\begin{enumerate}
% 		\item The unit: $K_1: 1 \hookrightarrow \w$
% 		\item The infinitesimals: $D: \wone^{op} \hookrightarrow \w$
% 		\item The finite-coproduct closure of infinitesimals $\{ \sum D_v | v \in \wone \} \hookrightarrow \w$ 
% 	\end{enumerate} 
% \end{example}
The category of finite sets is dense in $\s$, as $\s$ is locally finitely presentable and the finitely presentable sets are exactly finite sets. In particular, this means that the skeleton of finite sets, where each object is $[n] = \{1, \dots, n\}$, is dense in $\s$. The general idea of density as a generalization of this setting, and find the abstract notion of a Segal condition.
\begin{example}
    ~\begin{enumerate}[(i)]
        \item Consider a Lawvere theory $\th$, regarded as a cartesian category equipped with a bijective-on-objects, product-preserving functor $t:\mathsf{FinSet}_{\mathsf{skel}}^{op} \to \th$. Every object in $\mathsf{FinSet}_{\mathsf{skel}}$ is equivalent to a $[n] \cong \sum^n 1$. Then the category of models of $\th$ is equivalent to the pullback in $\mathsf{CAT}$:
        \[\input{TikzDrawings/Ch5/mod-of-th.tikz}\]
        \item Recall that the Segal condition states that a simplicial set $X$ is the nerve of a category if and only if each $X_n$ is the set of $n$-composible arrows of the underlying graph $s,t:X_1 \to X_0$. Now, recall that the category of graphs is exactly the category of presheaves over the free category generated by a pair of parallel arrows $s,t: 0 \to 1$, so any full subcategory of graphs containing $\yon 0, \yon 1$ is dense. We construct a dense subcategory of $\mathsf{Gph}$ where:
       \[ \input{TikzDrawings/Ch5/dense-in-graphs.tikz}\]
        so that $\mathsf{Gph}([n],G)$ picks out the set of paths of length $n$ in a graph $G$. We call this subcategory $P:\mathsf{Pth} \to \mathsf{Gph}$, and see that $N_P$ sends a graph to its $\mathsf{Pth}$-presheave of composible paths.
        Observe that we have a bijective-on-objects functor $t:\mathsf{Pth} \to \Delta$, so precomposition $t^*$ sends a simplicial set to the underlying $\mathsf{Pth}$-complex - the Segal conditions then state that the category of small categories is exactly the following pullback in the category of (possibly large) categories $\mathsf{CAT}$:
        \[\input{TikzDrawings/Ch5/pb-in-cat.tikz}\]
    \end{enumerate}
\end{example}


In the usual setting for Lawvere theories, the arities for our function symbols are given by natural numbers (e.g. finite sets), and the category of finite sets is a dense subcategory of $\s$. One can generalize this from $\s$ all the way to an arbitrary locally presentable $\vv$-category $\C$, where a dense subcategory $\a \hookrightarrow \C$ plays the role of the (skeleton of) category of finite sets. Power was the first to extend this to an arbitrary $\vv$-LFP $\C$, where the arguments for a Lawvere theory over $\C$ would then be the finitely presentable objects $\C_{fp}$. Berger-Mellies-Weber generalized this to dense subcategories of $\s$-LFPs $\C$, and Garner-Bourke's paradigm moved to dense sub-$\vv$-categories of LFP $\vv$-categories.

\begin{definition}%
    \label{def:nerve-theory}
	Let $K:\a \to \C$ be a dense $\vv$-subcategory of a locally finitely presentable $\c$.
    We call the replete image of $N_K$ in $\widehat{\a}$ the category of $K$-nerves.
	An \textit{$\a$-theory} is a bijective-on-object $\vv$-functor $J: \a \to \th$, where each
    \[
        \th(J-,a): \a \to \vv
    \]
    is a $K$-nerve.
	The category of concrete models for an $\a$-theory is given by the pullback in $\vv\mathsf{CAT}$:
    \[\input{TikzDrawings/Ch5/conc-models.tikz}\]
    We say that an $\a$-presheaf $X$ satisfies the $K$-Segal conditions whenever $t^*X$ is a $K$-nerve (that is, it is a concrete model of the theory).
\end{definition}
\begin{example}
    ~\begin{enumerate}[(i)]
        \item A functor $t:\mathsf{FinSet_{Skel}} \hookrightarrow \th$ is a $\mathsf{FinSet_{Skel}}$-theory if and only if $\th$ is a Lawvere theory. The Segal conditions in this case identify the models of the Lawvere theory.
        \item The inclusion of $\mathsf{Pth} \hookrightarrow \Delta$ is a $\mathsf{Pth}$-theory for the category of graphs. The Segal conditions in this case capture the classical Segal conditions for categories.
    \end{enumerate}
\end{example}
We do not need the full monad/theory correspondence from Bourke-Garner. However, the following is a useful result:
\begin{proposition}
    Let $K: \a \hookrightarrow \C$ be a dense $\vv$-subcategory, and $J: \a \to \th$ an $\a$-theory.
    The category of concrete models of $J$ is monadic over $\C$.
\end{proposition}
\begin{proof}
    This proof relies on a technical lemma - note that $N_K$ is fully faithful and monadic (as it is the inclusion of full reflective subcategory), and $J^*$ is monadic as $J$ is a bijective-on-objects functor. The pullback along $N_K$ will be fully faithful (as fully faithful functors are the right class of maps for the (bo,ff)-factorization system on $\vv$-categories). 
\end{proof}

This chapter makes use of enriched nerves in a few ways. First, this theory allows for the intuition of ``Segal conditions'' for involution algebroids to be made concrete, by exhibiting the category of involution algebroids as the category of models of a theory over the category of anchored bundles. Second, the Lie derivative from \cref{sec:linear-approx-of-a-cubical-object} may be exhibited as a nerve construction, this puts the Lie derivative into the domain of functorial semantics and in a presentable tangent category will guarantee the existence of a left adjoint - the \emph{realization} of the Lie algebroid. These results make use of the enriched perspective on tangent categories, explained below.

\section{Differential objects as enriched structures}%
\label{sec:diff-obs-enrichment}

Starting with differential bundles, note that a morphism $E \to TE$ is represented by a map:
\[
	\infer{\hat{\lambda}:D \to \C(E,E)}{\lambda: 1 \to \C(E, E^D)}
\]
The commutativity condition, then, is equivalent to asking that the following diagram commutes:
\[\input{TikzDrawings/Ch5/dbun-commutativity.tikz}\]
That is, $\hat{\lambda}$ is a semigroup morphism $D \to \C(E,E)$. 
In any cartesian closed category with coproducts, a semigroup may be freely lifted to a monoid using the "maybe monad" $(-) + 1$.
\begin{definition}
	Define the one-object $\w$-category $\Lambda$ to be given by the monoid 
	\[
		\infer{m: (D+1) \x (D+1) \to D+1}{D \x D + D + D + 1 \xrightarrow{(\iota_L\o m | \iota_L | \iota_L |\iota_R)} D + 1}
	\]
\end{definition}
\begin{lemma}
	The category of lifts in a tangent category $\C$ is isomorphic to the category of $\w$-functors and $\w$-natural transformations $\Lambda \to \C$.
\end{lemma}
\begin{proof}
	We check that a $\w$-natural transformation is exactly morphism of lifts $f: \lambda \to l$.
	Starting with the $\w$-naturality square:
    \[\input{TikzDrawings/Ch5/w-nat.tikz}\]
	Now, rewriting $D+1 \to \C(A,B)$ as a semigroup map $D \to \C(A,B)$, we have:
	\[
		\infer{
			\infer{ 
				1 \xrightarrow{Tf \o \lambda'}\C(A,TB) 
			}{ 
				1 \xrightarrow{(\lambda',f)} \C(A,TA) \x \C(A,B) \xrightarrow{1 \x T} \C(A,TA) \x \C(TA,TB) \xrightarrow{m_{A,TA,TB}} \C(A,TB)
			}}{	
			D \xrightarrow{(\lambda,f\o !)} \C(A,A) \x \C(A,B) \xrightarrow{m_{AAB}} \C(A,B)
		}
	\]
	similarly, we see the other path is exactly $l \o f$. So a $\w$-natural transformation is exactly a morphism of lifts.
\end{proof}
We may also see that there is a natural idempotent on the category of lifts in a tangent category $\C$, given by $p \o \lambda: (E,\lambda) \to (E,\lambda)$.
This idempotent has a natural representation in the monoid $\Lambda$ as the map $1 \xrightarrow{\iota_L \o 0} D + 1$.
In fact we note that this idempotent is an absorbing element of the monoid $D+1$, so for any $f:X \to D+1$, we have that $m(f,0\o !) = m(0\o !, f) = 0\o !$. 
A pre-differential bundle is exactly a lift with a chosen splitting of the natural idempotent $p\o\lambda$.
Way may take the idempotent splitting of $\Lambda$ and call it $\Lambda^+$, and observe that a predifferential bundle is exactly a functor $\Lambda^+ \to \C$.
\begin{definition}
	We define the $\w$-category $\Lambda^+$ to be given by the set of objects $\{0,1\}$ with hom-spaces:
	\begin{itemize}
		\item $\Lambda^+(1,1) = D+1$, otherwise $\Lambda^+(i,j) = 1$.
		\item $m_{111} = m, m_{i11} = \iota_L \o 0 \o !, m_{i0j} = !$
	\end{itemize}
\end{definition}
The following lemma lets us simplify the composition in $\Lambda^+$.
\begin{lemma}
	Associativity of composition in $\Lambda^+$ can be written by embedding each hom-space into $D+1$
	$\w$-category, where we use inclusions:
	\begin{gather*}
		\Lambda^+(0,0) = 1 \xrightarrow{\iota_L \o 0 \o !} D+1  \hspace{0.25cm}
		\Lambda^+(0,1) = 1 \xrightarrow{\iota_L \o 0 \o !} D+1  \\
		\Lambda^+(1,0) = 1 \xrightarrow{\iota_L \o 0 \o !} D+1  \hspace{0.25cm}
		\Lambda^+(1,1) = D+1 \xrightarrow{id} D+1  
	\end{gather*}
    \[\input{TikzDrawings/Ch5/assoc.tikz}\]
\end{lemma}
Basic facts about idempotent splittings yield the following theorem:
\begin{lemma}
	The category of pre-differential bundles is exactly the category of $\w$-functors $\Lambda^+ \to \C$. 
\end{lemma}
Now that we have exhibited pre-differential bundles as the category of $\C$-valued presheaves on $\Lambda^+$, it is straightforward to exhibit the category of differential bundles as a reflective subcategory of pre-differential bundles in $[\Lambda^+, \C]$.
\begin{proposition}
    The category of differential bundles in a locally finitely presentable tangent category $\C$ is a reflective subcategory of $[\Lambda^+, \C]$, and is therefore a locally finitely presentable tangent category.
\end{proposition}
\begin{proof}
    The category of pre-differential bundles in $\C$ is isomorphic to $[\Lambda^+, \C]$. 
    By \Cref{cor:idemp-dbun}, the category of differential bundles is isomorphic to the category of algebras for a canonical idempotent monad on $\C$, where a pre-differential bundle is sent to the $T$-equalizer: 
    \input{TikzDrawings/Ch5/reflector.tikz}
    This equalizer will always exist if $\C$ has equalizers, so this gives a left-exact idempotent monad on $[\Lambda^+, \C]$ whose algebras are differential bundles. 
\end{proof}
The notion of comodels for differential bundles is relatively underdeveloped.
Recall that because $(D+1, m', \iota_L)$ is a commutative monoid, there is a bijective correspondence between functors
\[
	\Lambda = \Lambda^{op} \Rightarrow \infer{\Lambda \to \C}{\Lambda^{op} \to \C}
\]
and this extends to pre-differential bundles due to basic facts about idempotent splittings.
In a cartesian category equipped with an infinitesimal object, we have an alternative presentation of pre-differential bundles.
When considering the dual of Rosicky's universality diagram, one finds a co-additive bundle structure.
\begin{lemma}
	Let $\C$ be a cartesian category with an infinitesimal object.
	\begin{enumerate}[(i)]
		\item A pre-differential bundle may be presented as a pair $(y:D \x A \to A, a:1 \to A)$ where $a \o ! = y(0\o !, id)$.
		\item If the following diagram is a pushout and pushout powers of $a$ exist, there is a commutative comonoid in $(1/\C, +_0, id_1)$.
            \[\input{TikzDrawings/Ch5/coadditivite-bundle.tikz}\]
	\end{enumerate}
\end{lemma}
\begin{proof}
	For the first part, note that this is exactly asking that $a$ splits the idempotent $y(0,id)$.
	For the second part, we induce co-addition using:
    \[\input{TikzDrawings/Ch5/induce-coadd.tikz}\]
\end{proof}

The notion of a \emph{comodel} of differential bundles is relatively underdeveloped, but will be useful for our purposes.
A codifferential bundle will determine a functor
\[
    Q: (\Lambda^{+})^{op} \to \C
\]
whose nerve will land in the category of differential bundles in $\wone$.
Because $D$ is a commutative cosemigroup, a codifferential bundle is still determined by a functor $\Lambda^+ = (\Lambda^+)^{op} \to \C$.
\begin{definition}
    Let $\C$ be a $\w$-category with copowers by representables.
    Then a codifferential bundle in $\C$ is exactly an object $Q$ equipped with an algebra:
    \[
        y:Q \cdot D \to Q
    \]
    that is associative with respect to the semigroup multiplication on $D$, and a chosen splitting of the idempotent 
    \[
        Q \xrightarrow{Q \cdot 0} Q \cdot D \xrightarrow{y} Q
    \]
    We require that the following diagram is a coequalizer:
    \[\input{TikzDrawings/Ch5/comodel-coeq.tikz}\]
\end{definition}
\begin{lemma}
    Every codifferential bundle in a $\w$-category with copowers by representables determines a nerve functor 
    \[
        N_Q: \C \to [\Lambda^+, \w]
    \]
    that sends any object $C$ to differential bundle in $\w$.
\end{lemma}
There is one construction in particular that will be useful later on:
\begin{lemma}
    Let $\C$ be a $\w$ category with copowers, coequalizers, and products.
    If $(y:Q \cdot D \to A, M)$ is a codifferential bundle, and $a:A \to A$ is an idempotent. Then the pushout:
    \[\input{TikzDrawings/Ch5/po-det-cobun.tikz}\]
    determines a codifferential bundle on $S$.
\end{lemma}
\begin{proof}
    Note that $D \x (-)$ is the copower by $D$ functor, and copowers preserve colimits, so we have the following morphism:
    \[\input{TikzDrawings/Ch5/induced-morphism.tikz}\]
    Associativity follows by couniversality. Idempotent splittings are coequalizers, so the triple exists.
    The commutativity of colimits ensures that the action $y^s$ is couniversal.
\end{proof}

Finally, we observe the following:
\begin{proposition}
    $\Lambda^+$ is a dense subcategory of differential bundles in $\w$. 
\end{proposition}


\section{Segal conditions for involution algebroids}%
\label{sec:revisiting-segal-conds}

In this section we revisit the ``Segal conditions'' for involution algebroids using the enriched categories perspective. 
There are three theories presented in this section - the theory of differential bundles, the theory of anchored bundles, and the theory of involution algebroids.
We can observe that:
\begin{enumerate}[(i)]
    \item The category of differential bundles in any tangent category with equalizers is a reflexive subcategory of a functor category.
    \item The category of anchored bundles is a full subcategory of the functors from the category of Weil algebras of width 1 (e.g. $\{ \N, T_n \}$). The Segal conditions for an anchored bundles is that its underlying pre-differential bundle (the precomposition functor $\Lambda^+ \to \wone^1$) is a differential bundle.
    \item The category of involution algebroids a full subcategory of  $\w$-functors $[\wone^3, \C]$, and it has Segal conditions for the width-three prolongations of anchored bundles. This will exhibit the category of involution/Lie algbebroids as monadic over the category of anchored bundles, which was first noticed in \cite{Kapranov2007}.
\end{enumerate}
% 
% \paragraph{Differential bundles as an enriched structure}
% We take an old fact about $M$-sets, and apply it to the enriched setting (and forget the unit axiom)

% \paragraph{Anchored bundles}
Recall that an anchored bundle is a differential bundle $(q:E \to M, \xi, \lambda)$ equipped with a linear morphism to $TM$.
That is to say, there is a natural transformation:
\[
    \input{TikzDrawings/Ch5/nat-trans-anc.tikz}
    \input{TikzDrawings/Ch5/nat-trans-anc-2.tikz}
\]
Note that the $TM$ is a limit, and has the universal property that for any $C$:
\[
    \C(C, TM) \cong \w(D, \C(C,M))    
\]
To construct a syntactic category for $\w$, then, we must augment $\Lambda^+$ so that the object $1$ is a cylinder for that limit diagram.
This agrees with previous results showing that the $\C$ is a reflective subcategory of the category of anchored bundles in $\C$, where $\rho$ acts as the reflector.
Recall that a cylinder for a diagram $G: \d \to \C$ weighted by $F:\d \to \w$ is given by an object $C$ and a $\w$-natural transformation:
\[
	F \Rightarrow \C(B, G-)
\]
so a cylinder for the tangent bundle of an object $C$ in $\C$ is given by the pair $K_D:1 \to \w, K_C: 1 \to \Lambda^+$, and the natural transformation is a map:
\[
	\infer{D \to \C(B,C) }{K_D \Rightarrow \C(B, C)}
\]
In the category $\Lambda^+$, we have $\Lambda^+(0,1) = 1$ so there is a unique cylinder
\[
	\w(D, \Lambda^+(0,1)) \cong \w(D, 1) = \{ !:D \to 1\}
\]
This corresponds with the linear morphism:
\[\input{TikzDrawings/Ch5/cor-to-lin-mor.tikz}\]
The category of \emph{truncated} Weil algebras solves this problem. 
\begin{definition}
    Define $\wone^1$ to be the full subcategory of $\wone$ spanned by $\{ \N, T \}$ (regarding $\wone$ as a $\w$-category).
\end{definition}
The object $T$ is a differential bundle in $\wone$, so we have there is a functor from $\Lambda^+ \to \wone^1$.
\begin{proposition}
    Every anchored differential bundle in $\C$ determines a functor $\wone^1 \to \C$, a natural transformation is exactly a tangent natural transformation.
\end{proposition}
\begin{proof}
    Start with an anchored bundle $(q:E \to M, \xi, \lambda, \anc)$. Then we have for hom-objects with domain $\N$:
    \[
        \wone^1(\N,\N) = 1 \mapsto id_M \hspace{0.5cm} \wone^1(\N,T) = 1 \mapsto \xi
    \]
    The hom-objects with domain $T$, the problem is slightly more difficult as $\wone^1(T,\N)(T^V) = \wone(T, T^V)$ and $\wone^1(T, T)(T) = \wone(T, T.T^V)$.
    This amounts to constructing maps:
    \[
         \wone(T, T^V) \to \C(E, T^V.M) \hspace{0.5cm}  \wone(T,T^V.T) \to \C(E, T^V.E)
    \]
    The first mapping is straightforward, send $f$ to $f.M \o \anc$. The second map relies on the fact that every map:
    \[
        T \to T^V
    \]
    in $\wone$ may be constructed using only $\{p,+,0,\ell\}$ closed under composition, pairing, and maps induced the universality $\ell$ (since there is only a single source variable).
    Thus for each $f:T \to T^V$ we can construct $f':E \to TE$ using $\{ q, +_q, \xi, \lambda\}$, pairing, and the universality of $\lambda$.

    The inclusion $\Lambda^+ \to \wone$ ensures that any tangent natural transformation will be a linear morphism on the underlying differential bundle, and the tangent natural transformations coherences ensures that a tangent natural transformation will preserve the anchor.
    Conversely, an anchored bundle morphism will preserve each of the constructed morphisms $E \to T^V.E, E \to T^V.M$ (as it preserves each of $\{ q, +_q, \xi, \lambda\}$), giving a tangent natural transformation. Thus there is a faithful embeddings $\mathsf{Anc}(\C) \hookrightarrow [\wone^1, \C]$.
\end{proof}

We use our first Segal condition. Observe that there is a bijective-on-objects functor
\[
    a: \Lambda^+ \to \wone^1
\]
The category $\Lambda^+$ is a dense subcategory of differential bundles, and each object $\N, 1$ have the structure of a differential bundle (e.g. they have a lift satisfying Rosicky's universality condition).
Thus we have the following:
\begin{lemma}
    The category $\wone^1$ is a $\Lambda^+$ theory on the category of differential bundles in $\w$.
\end{lemma}
The category of anchored bundles in $\w$ is precisely the category of presheaves on $(\wone^{1})^{op}$ whose underlying pre-differential bundle is a differential bundle. Thus we characterize the category of anchored bundles using the following pullback in $\w-CAT$:
\[\input{TikzDrawings/Ch5/anc-as-pb-in-cat.tikz}\]
That is, the Segal conditions for an anchored bundle is exactly a co-presheaf on $\wone^1$ whose underlying pre-differential bundle is a differential bundle.
\begin{proposition}
    The category of anchored bundles (in $\w$) is monadic over the category of differential bundles in $\w$.
\end{proposition}
For any tangent category $\C$, then, the following holds (using the embedding theorem).
\begin{corollary}
    For any tangent category $\C$, we have the following characterization of the anchored bundles in $\C$.
    \[\input{TikzDrawings/Ch5/anc-as-pb-in-cat2.tikz}\]
\end{corollary}


% \paragraph{Segal conditions for involution algebroids}
In order to give Segal conditions for involution algebroids, we must develop the appropriate set of arities.
This involves developing the \emph{coprolongations} of the initial co-anchored bundle given by $\yon: (\wone^1)^{op} \hookrightarrow \mathsf{Anc}(\w)$.

The idea of a coprolongation is to take the limit defining the $UV$-prolongation:
\[\input{TikzDrawings/Ch4/Sec3/span-comp.tikz}\]
and turn it into a representable functor $\mathsf{Anc}(\w) \to \w$.

\begin{definition}
    Let $(y:D \x A \to A, a:1 \to A, \delta: D \to A)$ be a co-anchored codifferential bundle. The coprolongation of $A$ by a Weil algebra $V$ is the cospan defined inductively by:
    \begin{enumerate}[(i)]
        \item $A(R): 1 \xrightarrow{=} 1 \xleftarrow{=} 1$
        \item $A(W^n):1 \xrightarrow{a(n)} A(n) \xleftarrow{\delta(n)} D(n)$
        \item $A(V \ox W^n)$ is given by cospan composition:
        \input{TikzDrawings/Ch5/cospan-comp.tikz}
    \end{enumerate}
\end{definition}

\begin{proposition}
    In the category of anchored bundles in $\w$, the representable functor:
    \[
        [\wone^1, \w](A_V, -)        
    \]
    sends an anchored bundle $B$ to its prolongation $\prol(V, B)$.
\end{proposition}
\begin{proof}
    This uses the Yoneda embedding, and the continuity of \[[\wone^1, \w](-, X): \mathsf{Anc}(\w) \to \w \] 
    This functor sends the diagram in question to the exact span composition defining the prolongation of the anchored bundle $X$.
\end{proof}

In the category of microlinear anchored bundles, there is the initial representable comodel given by the Yoneda embedding.
\[
	\yon(0) = 1, \yon(1) = L
\] 
For any anchored bundle $(\pi:A \to M, \xi, \lambda, \anc)$ in $\w$, the Yoneda lemma ensures that:
\[
	\mathsf{Anc}(\w)(1, A) = M, \mathsf{Anc}(\w)(L, A) = A
\]
so by the above proposition, we have $\mathsf{Anc}(\w)(L(V), A) = \prol(A, V)$.
This means that the category of ``prolongation complexes'' are naturally defined as presheaves on the coprolongations of $(y:D \x L \to L, 0, \delta)$ in $\mathsf{Anc}(\w)$.

\begin{definition}
	The $\w$-category ${\prol}$ is defined to be the full subcategory of $\mathsf{Anc}(\w)$ spanned by the coprolongations of the comodel $\yon:\wone^1 \to \mathsf{Anc}(\w)$.
\end{definition}


\begin{proposition}
	For any tangent category $\C$, there is a fully faithful inclusion:
	\[
		\mathsf{Anc}^*(\C) \to [{\prol}, \C]
	\]
	where $\mathsf{Anc}^*$ is the full subcategory of anchored bundles where all prolongations by $\wone$ exists.
\end{proposition}
\begin{proof}
	By the lemmas, we have that $\mathsf{Anc}(\w) \to [{\prol}, \w]$ is fully faithful.
	It then follows that the following functor is fully faithful:
	\[
		[\C^{op}, \mathsf{Anc}(\w)] \to [\C^{op}, [{\prol}, \w]]
	\]
	By the symmetry of theories, we can see that:
	\[
		\mathsf{Anc}(\widehat{\C}) \hookrightarrow [{\prol}, \widehat{\C}]
	\]
	Note that $\mathsf{Anc}(\C)$ is the full subcategory of $\mathsf{Anc}(\widehat{\C})$ where the anchored pre-differential bundle factors through the representables $\wone^1 \to \C \hookrightarrow \widehat{\C}$. 
	Because the inclusion $\C \to \hat{C}$ is flat, if an anchored bundle in $\C$ is complete then so to is its prolongation complex ${\prol} \to \widehat{C}$ factors through $\C$, so that we have the desired inclusion: 
	\[
		\mathsf{Anc}^*(\C) \to [{\prol}, \C]
	\]
\end{proof}

We finish by proving the main result in this section, that involution algebroids are models of a $\prol$-theory. 
The first step is giving a bijective-on-objects functor from the prolongation complex category and Weil algebras.
\begin{lemma}
	There is a bijective-on-object $\w$-functor ${\prol}^{op} \to \wone$.
\end{lemma}
\begin{proof}
	This follows from the dual result that $\w$ is a reflective subcategory of $\mathsf{Anc}(\w)$; we have that $\w$ is coreflective in the category of anchored codifferential bundles; the coreflector sends $L \mapsto D$, and so the pushouts $L(V) \mapsto D(v)$.
%	The trick here is to observe that $\w \hookrightarrow \mathsf{Anc}$ is a reflective subcategory of anchored bundles, sending an anchored bundle to its ``discrete'' anchored bundle $\lambda = \anc = 0:A \to TA$, and the coreflector sends $L(V) \mapsto D^V$.%TODO check this 
\end{proof}
\begin{proposition}
	Involution algebroids in $\w$ are models of the ${\prol}$-theory ${\prol} \to \wone^{op}$.
\end{proposition}
\begin{proof}
	The category of microlinear involution algebroids is exactly the category of cartesian models of $\wone$ in $\w$. 
	These are precisely the category of $\wone$-copresheaves where 
	\[
		(A.p,A.0, \alpha \o A.\ell, \alpha)
	\]
	are anchored differential bundles, where $A.T^U = \prol(A,U)$, which is the subcategory of $\widehat{\wone^{op}}$ that lands in the image of $\iota: \mathsf{Anc}(\w) \hookrightarrow \widehat\prol$.
\end{proof}
We can use embedding theorems and the symmetry of theories to show that the this holds more generally for the category of complete involution algebroids in any tangent category.
\begin{corollary}
	The category of complete involution algebroids in a tangent category $\C$ is precisely the pullback in $\w$-cat:
	\begin{equation}\label{eq:prol2}
        \input{TikzDrawings/Ch5/prol2.tikz}
	\end{equation}
\end{corollary}
\begin{corollary}
    The category of involution algebroids in a tangent category $\C$ is exactly the pullback:
    \begin{equation}\label{eq:prol3}
        \input{TikzDrawings/Ch5/prol3.tikz}
    \end{equation}
    where we write the category of width-three prolongations of an anchored bundle $\prol^3$.
\end{corollary}
In particular, this means that we can write the category of Lie algebroids as a pullback in $\w$-cat:
\begin{corollary}
	The category of Lie algebroids is the pullback in $\w\mathsf{Cat}$:
    \[\input{TikzDrawings/Ch5/lie-algd-monadic.tikz}\]
\end{corollary}
And finally, observe that in any locally presentable tangent category the category of involution algebroids is monadic over the category of anchored bundles, as previously observed in \cite{Kapranov2007}.
\begin{corollary}
	In a locally presentable tangent category $\C$, the category of involution algebroids is monadic over the category of anchored bundles in $\C$.
\end{corollary}

There are still some important properties to check in the category of involution algebroids. 
In any tangent category $\C$, the product in $[\wone,\C]$ of involution algebroids is an involution algebroid, so to show that $\mathsf{Inv}(\w)$ is a cartesian closed category, it suffices to show that it is an exponentiable ideal of $[\wone,\w]$ using the cartesian closed structure on $\w$-presheaves.
\begin{proposition}
	The category of involution algebroids in $\w$ is cartesian closed. 
\end{proposition}
\begin{proof}
	We need only show that involution algebroids are an exponential ideal in $[\wone,\w]$.
	This is equivalent to checking that for any involution algebroid $A$ and copresheaf $Q$, that $[Q,A](v)$ is the prolongation of the underlying anchored bundle.
	However, this follows as as simple calculation yields:
	\[
		[Q,A](v) = [\wone, \w](Q, [\yon (v), A])
	\]
	and $[\wone,\w](Q,-)$ is a $\w$-continuous functor, so it sends the limit defining $\prol(A,V)$ to the limit defining $\prol([Q,A],V)$.
%	\begin{align*}
%		[Q,A](v) &= [\wone, \w](Q \x \yon (v), A) \\
%				 &= [\wone, \w](Q, [\yon (v), A]) \\
%				 &= [\wone, \w](Q, \{ \prol_v, A\}) \\
%				 &= \{ \prol_v, [\wone, \w](Q, A) \}
%	\end{align*}
\end{proof}


\section{The infinitesimal nerve of a groupoid and its realization}%
\label{sec:inf-nerve-of-a-gpd}

The idea of this category is to construct a cartesian $\w$-functor:
\[
    \partial: \wone \to \mathsf{Gpd}(\w)    
\]
so that the nerve $N_\partial$ will coincide with the Lie functor from groupoids to algebroids. 
This has two major consequences, the first it equips the category of groupoids in $\mathsf{Gpd}(\w)$, and as a consequence the category of internal groupoids in most tangent categories, with a new tangent structure. The second consequence is that it puts the Lie functor into the nerve/realization paradigm, allowing for the construction of a groupoid from an algebroid.

% \paragraph{Revisiting groupoids and cubical objects}
Following \cref{sec:gpds-and-cub}, internal groupoids will be treated as a full subcategory of cubical objects. The language of locally presentable categories and density allows us to make simplify some of our previous results.
Recall that by \cref{prop:gpd-2cub-ff}: 
\begin{lemma}
    The arrow groupoid is a cubical monoid, and 2-truncation:
    \[
        \square_2 \hookrightarrow \square \xrightarrow[]{I} \mathsf{Gpd}
    \]
    is a dense functor.
    % \begin{enumerate}[(i)]
    %     \item $\square_2 \to \mathsf{Gpd}$
    %     \item $\square^{\mathsf{Conn}}_2 \to \mathsf{Gpd}$
    %     \item $\square^{\mathsf{SymConn}}_2 \to \mathsf{Gpd}$
    % \end{enumerate}
\end{lemma}
Now we can use the cancellativity result from \Cref{cor:dense-ff-result} to get the following:
\begin{proposition}%
    \label{prop:I-is-dense}
    The following functors arrow groupoid determines determiens a dense functor $\square \to \mathsf{Gpd}$.
\end{proposition}
\begin{proof}
    In every case, observe that the composite $\square_2 \hookrightarrow \square \to \mathsf{Gpd}$ is a dense functor, while the first map is fully faithful, thus the second map is a dense functor.
\end{proof}
This result was proved more concretely in \cref{cor:gpd-cub-ff}, but is a useful demonstration of density. 
\begin{corollary}
    The category of groupoids in $\w$ is a cartesian monoidal reflective subcategory of cubical objects in $\w$. 
\end{corollary}

Following the work in \Cref{sec:revisiting-segal-conds}, we wish to construct a cubical object that represents the linear approximation. Recall that given a cubical object $C$, the objects $C^\partial, C^{\partial \x \partial}, \dots$ are defined using $n$-fold equalizers:
\[\input{TikzDrawings/Ch5/nfold-eqs.tikz}\]
This is a cocomplete $\w$-category so the a cubical object $C \mapsto T.C.2$ is represented by $D \x I$. Thus, by taking the $n$-fold coequalizers:
\[\input{TikzDrawings/Ch5/nfold-coeq.tikz}\]
which is equivalent to the $n$-fold product of the equalizer diagram:
\[\input{TikzDrawings/Ch5/prod-coeqs.tikz}\]
the functor sending $C$ to $C^{n\cdot \partial}$ is represented by $n\cdot \partial$.
\begin{proposition}
    The object $\partial \cdot n$ is $n$-fold coequalizer:
    \[\input{TikzDrawings/Ch5/prod-coeqs.tikz}\]
    in cubical Weil spaces, and groupoids in $\w$.
\end{proposition}
\begin{proof}
    This follows from the fact that the category of cubical Weil spaces and groupoids in $\w$ are both cartesian closed, so that $(-) \x (-)$ is cocontinuous in each variable.
\end{proof}
The object $\partial$ is very nearly an infinitesimal object in the category of cubical Weil spaces.
\begin{definition}\label{def:structure-maps-del}
    Define the following maps on $\partial$.
    \begin{enumerate}[(i)]
        \item There is a point $0 \to \partial$ induced by:
        \[\input{TikzDrawings/Ch5/partial0.tikz}\]
        \item Write pushout powers of $0$ as $\partial(n)$. 
        \[\input{TikzDrawings/Ch5/delta-coadd.tikz}\]
        There is a map $\delta: \partial \to \partial(2)$ induced by:
        \[\input{TikzDrawings/Ch5/delta-coadd2.tikz}\]
        \item There is a cosemigroup structure $\odot: \partial \x \partial \to \partial$ induced by:
        \[\input{TikzDrawings/Ch5/cosemi.tikz}\]
        \item There is a co-anchor map $d:D \to \partial$ induced by the target:
        \[\input{TikzDrawings/Ch5/coanchor.tikz}\]
    \end{enumerate}
\end{definition}
\begin{lemma}%
\label{lem:structure-coherences}
    We have the following properties on $\partial$, where we write the pushout powers of 
    \begin{enumerate}[(i)]
        \item $\partial$ has a co-additive bundle structure $(0:1 \to \partial, !:\partial \to 1, \delta: \partial \to \partial(2))$, and $d$ preserves the co-addition.
        \item $\partial$ is a commutative semigroup with degeneracy $0$, and $d$ preserves the cosemigroup morphism and degeneracy.
        \item The following diagram commutes:
        \[\input{TikzDrawings/Ch5/coherence-for-structure-thing.tikz}\]
    \end{enumerate}
\end{lemma}
\begin{proof}
~\begin{enumerate}[(i)]
    \item This follows from co-associativity on $D$. Co-additivity of $d$ follows by precomposition:
    \input{TikzDrawings/Ch5/Coadditivity.tikz}
    \item The commutative cosemigroup axioms with degeneracy axioms all follow from the axioms on $D$. That $d$ is a cosemigroup homomorphism comes from precomposition (note that $I.\delta^+$ is the unit for $I.\gamma^+$)
    \input{TikzDrawings/Ch5/cosemigp.tikz}
    \item Consider the following diagram, where the maps into the center square are the relevent quotient maps.
    \input{TikzDrawings/Ch5/diag-commutes.tikz}
    The outer square commutes, and each of the maps commutes with the coequalizers diagrams. Thus, we may conclude that the center diagram commutes.
\end{enumerate} 
\end{proof}
\begin{proposition}
    The infinitesimal object $\delta$ represents the linear approximation functor $\widehat{\square^L} \to \w$.
\end{proposition}

So far we have represented the linear approximation functor, constructing an object that behaves like a Lie groupoid (but does not satisfy the necessary universality conditions). 
Recall that a cubical object with symmetric connections had an associated involution algebroid whenever the two morphisms:
\[
    z: C^{\partial \x \partial} \to \prol(C^\partial), \hspace{0.5cm}
    z_2: C^{\partial\x\partial\x\partial} \to \prol^2(C^\partial)
\]
are isomorphisms. 
We can formalize this as a natural transformation to the category of prolongations:
\[\input{TikzDrawings/Ch5/nat-in-prols.tikz}\]
Where:
\begin{enumerate}[(i)]
    \item The nerve $L$ refers to the functor $L: \prol \to \widehat{\square^L}$ induced by regarding $\partial$ as a co-anchored bundles and taking its coprolongations.
    \item The functor $Q^*$ identifies a functor from the full subcategory spanned by $\partial$ to the category $\prol$.
\end{enumerate}
\begin{proposition}
    The infinitesimal approximation object $\partial$ is a co-anchored bundle.
\end{proposition}
% \begin{proof}
%     The action is given by $y:D \x \partial \xrightarrow{} \partial \x \partial \to \partial$, and so it has the original unit $0:1 \to \partial$. %TODO this needs more
% \end{proof}

\begin{notation}
    Write the coprolongation of $D \to \partial$ as $L$, and more generally write the coprolongation of $\partial$ by the Weil algebra $V$ as $L_V$.
\end{notation}


\begin{proposition}
    There is a functor $Q:\prol \to \widehat{\square^L}$ that sends $v \mapsto \prol_v$, and a unique natural transformation:
    \[\input{TikzDrawings/Ch5/QFunct.tikz}\]
\end{proposition}
\begin{proof}
    The coprolongation defining $L_v$ has $\partial_v$ as a cocylinder, by observing that the following diagram commutes:
    \[\input{TikzDrawings/Ch5/coprol-inductive.tikz}\]
    and the result follows by induction.
\end{proof}

\begin{definition}
    A microlinear cartesian cubical object is a \emph{local groupoid} precisely whenever the map $z^*: N_Q(C) \to N_L(C)$ is an isomorphism.
\end{definition}
\begin{proposition}
    In the category of local groupoids, $\partial$ is an infinitesimal object. 
    (In this case, we mean the appropriate limit computing $\partial$ in the infiniteismal objects).
\end{proposition}
\begin{proof}
    The only axiom that fails for $\partial$ in the category of cartesian cubical objects in $\w$ was the universality of the vertical lift. 
    However, we have that the diagram:
    \[\input{TikzDrawings/Ch5/couniversal-colift.tikz}\]
    is a coequalizer for every cubical object, and this diagram corresponds to the coequalizer:
    \input{TikzDrawings/Ch1/InfObj/coeq.tikz}
\end{proof}
\begin{corollary}
    The category of local groupoids has a tangent structure that is represented by $\partial$.
\end{corollary}
Returning to \Cref{sec:linear-approx-of-a-cubical-object}, the result \Cref{prop:gpd-is-local-gpd} guarantees that groupoids are local groupoids.
Thus the following holds:
% \begin{proof}
%     We use that groupoids are an exponential ideal, and we have shown in the original treatment of groupoids that $[L_{WW},G] \cong [\partial \x \partial, G]$ - applying this fact inductively yields the result. More concretely, just consider 
% \end{proof}


\begin{theorem}[The infinitesimal nerve]
    In the category of (local) groupoids in $\w$ has a $\w$-functor $\partial: \wone \to \mathsf{LocGpd}$, and the nerve of $\partial$ factors through the category of involution algebroids.
    \[\input{TikzDrawings/Ch5/inf-nerve.tikz}\]
\end{theorem}
\begin{corollary}
    Note that a (local) groupoid in the category of $\w$-presheaves on $\C$ may be regarded as a $\w$-functor from $\C$ into the category of (local) groupoids. Similarly, an involution algebroid in the category of $\w$-presheaves on $\C$ may be regarded as a $\w$-functor $\C \to \mathsf{Inv}(\w)$.
    The infinitesimal nerve agrees with the Lie functor - that is to say, the following diagram commutes:
    \[\input{TikzDrawings/Ch5/inf-nerve-commutes.tikz}\]
\end{corollary}

\begin{observation}
    Note that the object $\partial_V$ in $\mathsf{LocGpd, Gpd}$ is constructed as a finite colimit of representable objects.
    This means, in particular, that the $\partial_V$ is a finitely presentable object, so that is is a co-model of $\mathsf{Inv}$ in the category of finitely presentable objects in $\mathsf{LocGpd, Gpd}$.
    This induces left-exact $\w$-morphisms from $\mathsf{Inv}_{fp}^{op} \to \mathsf{Gpd}_{fp}^{op}$, exhibiting the Lie functor as pre-composition (so it is induced via the Gabriel-Ulmer syntax/semantics adjunction).
\end{observation}
% This ends up making use of a fairly obscure technical condition on $\s$, that we can then extend to cartesian cubical objects and then microlinear groupoids.
% \begin{proposition}
%     % In the category of microlinear cartesian cubical objects, and microlinear groupoids, pushouts of the following form are 
%     In any cartesian monoidal reflective subcategory of a pre-sheaf tangent category, pushouts of the form:

%     are closed under products.
% \end{proposition}
% \begin{proof}
    
% \end{proof}
% \begin{corollary}
%     The $\partial^n$ is the colimit of the $n$-fold coequalizer:

% \end{corollary}





% \begin{proposition}
%     Write the arrow groupoid $I$. The full category spanned by $I$ in $\mathsf{Gpd}(\s)$ is dense.
% \end{proposition}
% \begin{proof}
%     Recall that for the construction of the cubical object of a groupoid, we had $G_n = \mathsf{Gpd}(\s)(I^n, G)$. 
%     This means that the functor $I^{(-)}: \square_{\mathsf{SymCon}} \to \mathsf{Gpd}(\s)$ is dense, and by -, this factors as two dense functors.%Add this lemma
%     This means that the full subcategory of $\mathsf{Gpd}(\s)$ spanned by $I^n$ is dense.
% \end{proof}
% \begin{corollary}
%     Consider the free Lawvere theory generated by the structure maps of a cubical monoid
%     %TODO include diagram here
%     satisfying the necessary maps (note that in this case, $\epsilon$ is now $!$). 
%     We call this the cartesian cube category $\square_{\mathsf{Cart}}$ and call the corresponding category of presheaves the category of cartesian cubical set,.
%     Observe the arrow groupoid $I$ is a model of this Lawvere theory.
%     Now use the the cancellation for dense functors from ,%TODO add reference
%     We can see that the category of internal groupoids is a full subcategory of the category of cartesian cubical sets.  
% \end{corollary}
% \begin{corollary}
%     The category of microlinear groupoids is cartsian closed, as it is a reflective subcategory of cartesian cubical sets. 
% \end{corollary}

% \begin{corollary}
%     The category of microlinear groupoids (e.g. groupoids in $\w$) is a reflective sub-tangent-category of $\widehat\square^{\mathsf{Cart}}$, where we treat $\square^{\mathsf{Cart}}$ as a trivial $\w$-category.
% \end{corollary}

% We begin by constructing an object $\partial$ that represents the $C^\partial$ construction from the previous chapter.
% \begin{definition}
%     Define the cartesian cubical object: $\partial(n)$ to be $\dots$ 
% \end{definition}
% \begin{proposition}
%     The object $\prod \partial(n_k)$ represents the functor blah
% \end{proposition}

% Now, we also note that $\partial$ acts as a co-differential bundle under $1$.
% \begin{itemize}
%     \item There is an action:
%     \item The action splits as:
%     \item There is a co-anchor:
% \end{itemize}
% Thus, we can construct the coprolongations of $\partial$, and write these $L_V$.
% \begin{definition}
%     The in the category of microlinear cartesian cubical objects, we have the object $L_V$ given by
% \end{definition}

% %TODO something about the d maps.

% \begin{proposition}
%     $\partial$ is an infinitesimal object.
% \end{proposition}

% \begin{proposition}
%     Each $\partial_v$ represents the functor $\prol(V,-)$.
% \end{proposition}


\section{The realization of the infinitesimal nerve}%
\label{sec:realization-of-inf-nerve}

As the final new result of this thesis, we construct an adjunction between (local) groupoids and involution algebroids in $\w$ using the nerve/realization paradigm. This adjunction is well-behaved: it is stable over the base-space of the cubical 

\begin{definition}
	Let $K: \D \to \C$ be a $\vv$-functor from a small $D$ into a cocomplete $\C$.
	The \textit{realization} of $K$ is the left adjoint to the $K$-nerve $N_K$, constructed as the following left Kan extension:
    \[\input{TikzDrawings/Ch5/real-kan-ext.tikz}\]
\end{definition}
\begin{lemma}
	The $K$-realization may be constructed as the following coend:
	\[
		|A|_K = \int^{D \in \D} A(V) \bullet K(V)
	\]
	where $A(V) \bullet(-)$ denotes the copower by the object $A(V)$ in $\w$.
\end{lemma}
We have constructed a $\w$-functor $\partial: \wone^{op} \to \mathsf{Gpd}(\w)$ that represents the $U$-approximation functor from groupoids into $\w$, so that the the nerve lands in involution algebroids. If we consider the Yoneda embedding of $\wone^{op}$ into the category of involution algebroids in $\w$, each $V$ determines a model $\delta^V$, and this $\delta^V$ represents the ``evaluate at $V$'' functor (so that it picks out the representables for the \textit{Lie} tangent structure). 
\[\input{TikzDrawings/Ch5/lie-tang.tikz}\]

The realization itself is computed as a coend - this has the funny effect that we are using the coend calculus integral to denote what (one hopes to be) the Lie integration functor :
\[
	|A|_\partial = \int ^{v \in \wone} A(v)\bullet \partial v 
\]
We see that for any groupoid $G$ and involution algebroid $A$:
\begin{align*}
	\mathsf{Gpd}(\w)(|A|_\partial, G)
	&= \mathsf{Gpd}(\w)(\int ^{v \in \wone} A(v)\bullet \partial v, G) \\
	&= \int_{v \in \wone} \mathsf{Gpd}(\w)( A(v)\bullet \partial v, G) \\
	&= \int_{v \in \wone} \w(A(v), \mathsf{Gpd}(\w)( \partial v, G)) \\
	&= \int_{v \in \wone} \w(A(v), N_{\partial}(G)(v)) \\
	&= [\wone,\w](A, N_{\partial}(G))
\end{align*}
All that remains to show is that $|-|_\partial$ is fully faithful - this requires a more careful analysis of the realization functor.
\begin{lemma}
	The realization functor preserves products.
\end{lemma}
\begin{proof}
	This is a consequence of the fact that $|-|_\partial$ is the left Kan extension of a cartesian functor along a cartesian functor.
	Note that this means $\int^v\partial(v) = 1$.
\end{proof}

\begin{lemma}\label{lem:base-of-groupoid}
	The base space of the groupoid $\partial$ is $D^v$.
\end{lemma}
\begin{proof}
	When constructing the colimit of groupoids, the colimits base space is constructed as the ordinary colimit for the diagram of the base spaces.
	The reflector from simplicial objects to groupoids preserves products, so it suffices to check that the base space of $\partial(n)$ is given by $D(n)$.
	
    The base space of $I$ is $1+1$, as:
    \[
        I(0) = \widehat{\square}(1,I) \cong \square(0,I) = 1 + 1
    \]
    and the map $e^-_0$ is given by $\delta^- \o !$. 
    $D$ is a discrete cubical object, so the base space is $D \x 1$.
    Thus the coequalizer defining $\partial$ is:
    \[\input{TikzDrawings/Ch5/coeq-def-partial.tikz}\]
    A map $\gamma: D + D \to M$ is a pair of maps $\gamma_0, \gamma_1: D \to M$. 
    We can see that $\gamma_0, \gamma_1$ agree at $0$ (they are both $\gamma_0(0)$), and $\gamma(0)$ is a constant tangent vector. It follows then, that $\gamma_1 \o (id | id) = \gamma$.
    % This result holds as a consequence of microlinearity. 
    % Note that $\square(0,1) = \{ \delta^\pm \}$, so $e^-$ sends $
	% The groupoid $D(n)$ is discrete, and the base space of $\yon(n)$ is $n\bullet 1 = \coprod_n 1$.
	% The diagram becomes:
	% \begin{equation*}
	% 	\begin{tikzcd}
	% 		(1 \x D(n)) + 2 \rar{(\iota_L \x 1 | 2\bullet 0)} \dar{((1\x !) | (id | id)) } &[3em] 2 \x D(n) \dar \\
	% 		1 \rar & (\partial(n))_0 
	% 	\end{tikzcd}
	% 	\cong
	% 	\begin{tikzcd}
	% 		D(n) + 2 \rar{i_L + (2\bullet0)} \dar[swap]{!} &[3em] D(n) + D(n) \dar \\
	% 		1 \rar & (\partial v(n))_0 
	% 	\end{tikzcd}
	% \end{equation*}
	% Now, we claim the following diagram is a pushout:
	% \begin{equation*}
	% 	\begin{tikzcd}
	% 		D(n) + 2 \rar{i_L + (2\bullet0)} \dar[swap]{!} &[3em] D(n) + D(n) \dar{(0! | id)} \ar[bend left]{rdd}{\gamma} \\
	% 		1 \rar{0} \ar[bend right]{rrd}[swap]{x} & D(n) \ar[dashed]{rd}{\gamma \o \iota_R} \\
	% 		& & X
	% 	\end{tikzcd}
	% \end{equation*}
	% First, notice that $\gamma$ is a pair of tangent vectors on $X$, and look at each injection into $D(n) + 2$.
	% \[
	% 	\gamma \o (i_L + (2 \bullet 0)) \o \iota_L = \gamma \o \iota_L, 
	% 	\hspace{0.3cm}
	% 	\gamma \o (i_L + (2 \bullet 0)) \o \iota_R = \gamma \o (2 \bullet 0)
	% \]
	% We can see that each tangent vector $\gamma \o \iota_L, \gamma \o \iota_R$ has the same base point, $x$.
	% \[ \gamma \o \iota_L \o 0 = \gamma \o (2 \bullet 0) \o \iota_L = x\o ! = \gamma \o (2 \bullet 0) \o \iota_R = \gamma \o \iota_R \o 0\]
	% Next observe that $\gamma \o \iota_L$ must be a constant tangent vector, as:
	% \[
	% 	\gamma \o \iota_L = \gamma \o (\iota_L + (2 \bullet 0)) \o \iota_L = x \o ! \o \iota_L = x \o !
	% \]
	% in particular, we have that $\gamma \o \iota_L = \gamma \o \iota_R \o 0 \o !$, 
	% so then a pair $(x,\gamma)$ uniquely determines a $D(n)$-tangent vector $\gamma \o \iota_R$.
%	%TODO uniqueness?
%	
%	{\color{red} I think this proof shows that this is a pushout in the entire presheaf category, since microlinearity on $X$ is never used}.
\end{proof}

%\begin{remark}
%	By the same argument as the lemma, we have
%	\begin{equation*}
%		\begin{tikzcd}
%			D^V + (n+1) \rar{i_0 + ((n+1)\bullet0)} \dar[swap]{!} &[3em] (n+1)\bullet D^V \dar{(0! | id)} \ar[bend left]{rdd}{\gamma} \\
%			1 \rar{0} \ar[bend right]{rrd}[swap]{x} & D^V(n) \ar[dashed]{rd}{\gamma \o \iota_R} \\
%			& & X
%		\end{tikzcd}
%	\end{equation*}
%	Therefore, we have that the simplicial object representing $\partial_V$ is given by:
%	\[
%		n \mapsto D^V(n)
%	\]
%	and because groupoids are a reflective subcategory of simplicial objects, we may compute
%	\[
%		[\partial^V, G](n) = [\Delta^{op},\w](\hat{\partial}^V \x \yon(n),G)
%	\]
%	However, it suffices for our purposes to have the base space characterized.
%\end{remark}

Now, recall the co-Yoneda lemma, for any $\vv$-presheaf $A: \C^{op} \to \vv$
\[
	F(C) = \int^{C' \in \C} \C(C,C') \ox F(C')
\]
so in particular, for an involution algebroid in $\w$ (or any $\w$-presheaf on $\wone^{op}$)
\[
	A(U) = \int^{V \in \wone} \wone^{op}(U,V) \x A(V) = \int^{V \in \wone} \wone(V,U) \x A(V) 
\]
\begin{lemma}\label{lem:as-a-presheaf}
	For any involution algebroid $A$:
	\[ A(R) = \int^{V \in \wone} A(V) \x D^V \]
\end{lemma}
\begin{proof}
	Use the tangent structure on $\wone$ to regard it as a $\w$-enriched category:
	\begin{gather*}
		D^V = \yon(V) = \wone(V,-) = (U \mapsto \wone(V, U))  \\= (U \mapsto \wone(V, U\ox R)) = \wone(V,R)
	\end{gather*}
	so that we may compute:
	\[
		A(R) = \int^{V} \wone(V,R) \x A(V) = \int^{V} D^V \x A(V) 
	\]
\end{proof}
This allows us to relate the base space of an involution algebroid and its associated groupoid. 

\begin{proposition}\label{prop:lie-int-first-part}
	Let $A$ be an involution algebroid in $\w$. Then $|A|([0]) = A(R)$.
\end{proposition}
\begin{proof}
	Use the Yoneda lemma, and that $\yon[0] = 1$ is a small projective so $\mathsf{Gpd}(1,-)$ is $\w$-cocontinuous, then apply \cref{lem:base-of-groupoid} and \cref{lem:as-a-presheaf}
	\begin{align*}
		|A|([0])&= \mathsf{Gpd}(1, |A|) \\
			    &= \mathsf{Gpd}\left(1, \int^{v \in \wone} A(v)\bullet \partial v \right) \\
			    &= \int^{v} A(v)\x \mathsf{Gpd}(1,  \partial v ) \\
			    &= \int^{v}  A(v)\x D^v = A(R)
	\end{align*}
\end{proof}

Note, then, there are two tangent structures on each of the category of (local) groupoids and the category of involution algebroids $\w$.
In order to prove that the realization functor into (local) groupoids is a coreflection, it would suffice to prove that the realization functor is a tangent functor for the second tangent structures, as:
\[
    \left(T_v(|A|) = [\partial_v, |A|] = |[\partial_v,A]| \right) \Rightarrow 
    \left(\mathsf{LocGpd}(\partial_v, |A|) = A(v)\right) \Rightarrow
    N_\partial(|A|) \cong A
\]
% This is equivalent to asking that the coend commute with the following pullback:
% \[
%     \int^v A(wv)\cdot \partial_v \cong \int^v (A(v) \ts{}{} T^v.A(w) ) \cdot \partial_v
%     \cong \int^v (A(v) \cdot \partial_v)\ts{\anc'}{T^v.\pi} (T^v.A(w)\cdot\partial_v)
% \]
%\begin{lemma}
%	There is a functor $\wone \to \w$ defined:
%	\[
%		v \mapsto \coprod^{\dim(v)} 1
%	\]
%	This is an involution algebroid, and its realization is the terminal groupoid.
%\end{lemma}
%\begin{proof}
%	
%\end{proof}
%
%\begin{proposition}
%	Any differential object, when regarded as an abelian involution algebroid, integrates to the pair groupoid.
%\end{proposition}
%\begin{proof}
%	\begin{align*}
%		|V|(2) &= \mathsf{Gpd}(\yon 2, |V|) \\
%			   &= \mathsf{Gpd}(\yon 2, \int^{u} T^uV \cdot \partial v ) \\
%			   &= \mathsf{Gpd}(\yon 2, \int^{u} V(R) \cdot [\dim(v)] \cdot \partial v ) \\
%			   &= \mathsf{Gpd}(\yon 2, V(R) \cdot \int^{u} [\dim(v)] \cdot \partial v ) \\
%			   &= V(R) \cdot \mathsf{Gpd}(\yon 2,  \int^{u} [\dim(v)] \cdot \partial v ) \\
%			   &= V(R) \cdot 2
%	\end{align*}
%\end{proof}

% \paragraph{How is the realization related to Lie integration?}
% {\color{blue}
% 	It is still unclear how Lie integration is related to this adjunction. 
% 	In particular, we may write the comonad on smooth groupoids as:
% 	\[
% 		S(\g) = \int^{v \in \wone} G.K(V) \cdot K(v)	
% 	\]
% 	where we observe that as each $\partial v$ is finitely presentable, we may factor our map as: 
% 	\[K: \wone \hookrightarrow \mathsf{Gpd}_{fp}^{op} \hookrightarrow \mathsf{Gpd}\]
% 	So, if we restrict our attention to the idempotent core of the adjunction, we have the counit $\epsilon$ is an isomorphism if and only if:
% 	\[
% 		\int^{v \in \wone} G.K(v) \cdot K(v) = \int^{v \in \mathsf{Gpd}^{op}_{fp}}G(v) \cdot \hat{v}
% 	\]
% }


% \end{document}
